When Can Liquid Democracy Unveil the Truth?

In this paper, we investigate the so-called ODP-problem that has been formulated by Caragiannis and Micha [10]. Here, we are in a setting with two election alternatives out of which one is assumed to be correct. In ODP, the goal is to organise the delegations in the social network in order to maximize the probability that the correct alternative, referred to as ground truth, is elected. While the problem is known to be computationally hard, we strengthen existing hardness results by providing a novel strong approximation hardness result: For any positive constant $C$, we prove that, unless $P=NP$, there is no polynomial-time algorithm for ODP that achieves an approximation guarantee of $\alpha \ge (\ln n)^{-C}$, where $n$ is the number of voters. The reduction designed for this result uses poorly connected social networks in which some voters suffer from misinformation. Interestingly, under some hypothesis on either the accuracies of voters or the connectivity of the network, we obtain a polynomial-time $1/2$-approximation algorithm. This observation proves formally that the connectivity of the social network is a key feature for the efficiency of the liquid democracy paradigm. Lastly, we run extensive simulations and observe that simple algorithms (working either in a centralized or decentralized way) outperform direct democracy on a large class of instances. Overall, our contributions yield new insights on the question in which situations liquid democracy can be beneficial.

==> Observations.tex <==
\section{Some Observations}\label{secobs}

A problem is called fixed parameter tractable (FPT) with fixed parameter $k$ and instance $I$ if it is solvable by an algorithm whose complexity is $O(f(k)|I|^{c})$, where $f$ is an arbitrary function depending only on $k$ and $c$ is a constant.
\begin{theorem}
Given a graph $G=(E, V)$. ODP is FPT w.r.t. $|E|$.
\begin{proof}
We can easily propose a brute-force method as an FPT algorithm to ODP: try all $\binom{E}{S}$ subsets $S$ of $E$ implying all delegation graphs in $\Delta(G)$ and return the subset $S$ that results in the highest chance of having T as the winner. Recall that for every delegation graph in $\Delta(G)$, the recursive formula~\ref{lbrecursiveformula} computes the probability of electing T in polynomial time. Hence the complexity of the FPT algorithm is $O(2^{|E|}n^{2})$, where $n=|V|$. Note that we can use the breadth-first search
technique to find out whether a subset $S$ of $E$ implies a delegation graph.
\end{proof}
\end{theorem}

To propose an efficient algorithm, we examine $k$-ODP in more detail and study what factors can have influence on $P_{H,\vec{p}}(T)$. In $k$-ODP, delegations partition a graph (social network) into some directed trees that are rooted at some gurus (if you reverse the delegation arcs). So, each guru takes this responsibility to vote for every follower in her corresponding tree. More formally, we are given a forest $\Forest = \{t_1,\ldots,t_q\}$, where $t_1,\ldots,t_q$ are the trees induced by $H$. We denote the guru of tree $t_i \in \Forest$, and the probability she casts a vote for T by $Gu(t_i)$ and $P(t_i)$ (i.e., $P(t_i)=P(Gu(t_i))$), respectively. We denote by $V_{t_i}$ and $E_{t_i}$ the set of nodes and arcs in $t_i$ respectively. Each $t_i$ is assigned a weight $w(t_i) = |V_{t_i}|$ (i.e., the voting power $Gu(t_i)$ receives from herself and her followers). We also extend this notation to subsets of trees by letting $w(a) = \sum_{t\in a} w(t)$, where $a\subseteq \Forest$. Let $A = \{ a\subseteq \Forest | w(a) \ge (n+1)/2\}$ be the set of all subsets of $\Forest$ which have enough weight to win the election. 
We denote the probability that the gurus voting for $T$ are exactly the ones corresponding to the subset $a$ by $ P(a)=\prod_{t \in a}P(t) \prod_{t \notin a} (1-P(t))$. 
As a result, $P_{H,\vec{p}}(T)$ can be rewritten as follows: 
$$P_{H,\vec{p}}(T) = \sum_{i=1}^{|A|} P(a_i).$$

Recall that our goal is to change at most $ k $ delegations in the set $\Forest$ in order to find another forest $\Forest^{'}$ that can detect the ground truth more efficiently.

To be on the right track, we first mention what factors effect the accuracy of outcome and then explain how they can change the result of voting. By using the following examples, we show that the probability of selecting the ground truth depends on two factors: the probability $P(t_i)$ and weight $w(t_i)$ of each tree $ t_i $ (i.e., the structure of $ H $).

\begin{exmp}\label{ex1}
	Fig.\ref{sn1} displays a SN, the competence levels of the voters which are given next to the corresponding nodes and a delegation graph. We have a budget $ k=2$, which means that we can change at most $ 2 $ delegations.
	%\ Every voter $ i \in \left\lbrace 1, 2, ..., 5 \right\rbrace  $ has competency level $ p_i $, indicating the probability that she will cast a vote for T when she votes directly. 
	Based on this social network, we show one of the possible delegation graphs in Fig.\ref{dg11}, in which voter 2 votes resulting in a decrease of the weight of voter 4. Under these modifications, we find that the ground truth is selected more likely.
	
	\begin{figure}[htbp]
		\centering
		
		\subfloat[The SN]{ \includegraphics[height=2.5cm,width=4cm]{figures/sn1.png}}\hspace{2cm}
		\subfloat[A delegation graph $H$ with $P_{H,\vec{p}}(T) = 0.74$.]{\label{dg1}\includegraphics[height=2.5cm,width=4cm]{figures/dg1.png}}
		\caption{}\label{sn1}
		%\label{fig:1}
	\end{figure}
	
	\begin{figure}[htbp]
		
		\centering
		\includegraphics[scale=.2]{figures/dg11.png}
		\caption{ $P_{H^{'}, \vec{p}}(T)= 0.795$.}\label{dg11}
		
		
		%\label{fig:1}
	\end{figure}
	
\end{exmp}

\begin{exmp}\label{ex2}
	Fig.\ref{sn2} displays the same SN with different competence levels and the same delegation graph.
	%\ Every voter $ i \in \left\lbrace 1, 2, ..., 5 \right\rbrace  $ has competency level $ p_i $, indicating the probability that she will cast a vote for T when she votes directly. 
	Fig.\ref{dg2} shows that in this case decreasing $ w(4) $ by making voter 2 vote directly has a negative effect on $P_{H,\vec{p}}(T)$.
	
	\begin{figure}[H]
		
		\centering
		\subfloat{\includegraphics[height=2.5cm,width=4cm]{figures/sn2.png}}\hspace{2cm}
		\subfloat{\includegraphics[height=2.5cm,width=4cm]{figures/dg2.png}}\label{2}
		\caption{ The SN, a delegation graph with $P_{H,\vec{p}}(T) = 0.98325$.}\label{sn2}
		%\label{fig:1}
	\end{figure}
	
	\begin{figure}[htbp]
		
		\centering
		\includegraphics[scale=.2]{figures/dg21.png}
		\caption{ $P_{H^{'}, \vec{p}}(T) = 0.9811$.}\label{dg2}
		
		
		%\label{fig:1}
	\end{figure}
	
\end{exmp}

These observations have motivated us to pay more attention to these two factors and their influence on $P_{H, \vec{p}}(T)$. For this purpose, we further investigate how changing a delegation affects the forest induced by the delegation graph $H$. In particular, by changing a voter's delegation, one of the following three actions can happen:

\begin{enumerate}
	\item $ Join $: this action takes two trees $ t, t' \in \Forest$ and returns a new tree $Join(t, t') = t \cup t'$ such that $Gu(Join(t, t')) = Gu(t)$. Note that $Join(t, t')$ is different from $Join(t', t)$. %\HG{It is not clear that where you make the Join has an impact or not on the algorithm.(?)}
	
	\item $Split$: this action takes a tree $ t \in \Forest $, and a voter $i \in t$ such that $i\neq Gu(t)$ and partitions $t$ into two trees $t_i, t_{\overline{i}}$, such that $t_i$ is the subtree of $t$ rooted in $i$ and $t_{\overline{i}} = t\setminus t_i$ .
	%denoted by $\Forest_t$, where $|V_{t_i^{'}}|\ge 1$ and $|V_{t_j^{'}}|\ge 1$ ($\Forest_t=Split(t)$). For the sake of simplicity, we suppose $ Gu(t_i^{'})=Gu(t) $, and so $P(t_i^{'})=P(t)$.
	
	\item $ ReDelegate $: this action takes as input a tree $ t \in \Forest $, and a voter $i \in t' \neq t$ such that $i \neq Gu(t')$ and is equivalent to first performing $Split(t',i)$, and then performs $ Join(t, t_i)$.
	%for all possible $t_j^{'} \in \Forest_t$ and trees $ t_j \in \Forest\setminus \left\lbrace t_i \right\rbrace  $, which is its current guru. In other words, $ ReDelegate(t) = Join(Split(t), t_j), \forall t_j \in \Forest \setminus \left\lbrace t_i \right\rbrace$.
	
	
\end{enumerate}


As it can be seen, in Examples~\ref{ex1} and \ref{ex2}, an action may increase or decrease the probability of a subset $a_i$. In the following, we examine how these actions can effect the outcome of election in more detail, which helps us to prove some interesting results, especially helps us to bound the optimal solution later in this study. Consider tree $ t \in a_i \subseteq A$. Let $t_i$ and $t_{\overline{i}}$ be the outcome of $Split(t, i)$ and $a^{'}_i = a_i\cup\{t_i\}\setminus t$ and $a^{'}_{\overline{i} }= a_i\cup\{t_{\overline{i}}\}\setminus t$. Let $ P(a^{'}_i) $ and $ P(a^{'}_{\overline{i}}) $ be the probability that $a^{'}_i$ and $a^{'}_{\overline{i}}$ votes for T after performing $Split(t)$, respectively.\footnote{Or $Join$ or $ ReDelegate $} We bellow show that partitioning $ t $ may have different (positive or negative) influence on $ P_{H,\vec{p}}(T)$.\footnote{ To show how joining a subset of trees has effect on discovering the ground truth, we can go in opposite direction. Also, the combination of $ Join $ and $Split$ help us to analyze $ ReDelegate$.} In particular, with respect to $ P(a_i) $, in the following possible value of $ P(a^{'}_i) $ and $ P(a^{'}_{\overline{i}})$ are examined. %\HG{All this part is problematic. \(a_i\) is not well defined after the split. Let's call it \(a_i'\). Is $a_i = a_i\cup\{t_i^{'}, t_j^{'}\}\setminus t$? All the items below seem false to me because $P(a_i)$ does not correspond to the definition it had before. Moreover, $ P_{H,\vec{p}}(T)$ is a sum of $P(a_i)$ values whose number of summands increases after the split. This seems not to be taken into account in your analysis. }

%\begin{enumerate}
%\item If $w(a_i) \ge \dfrac{n+1}{2}$ when either $Gu(t_i)$ votes for T or F \HG{$w(a_i)$ does not depend on the vote of $Gu(t_i)$ so I don't understand what you mean.}, $ P^{'}(a_i) =P(a_i)$.

%Recall that, $w(a_i) \ge \dfrac{n+1}{2}$ when $Gu(t_i)$ should vote for T, the following cases can happen.

\begin{enumerate}
	\item \label{case2.1} If both $ Gu(t_i)$ and $ Gu(t_{\overline{i}})$ should vote for T (i.e., $w(a_i)-w(t)+w(t_i)< \frac{n+1}{2}$ and $w(a_i)-w(t)+w(t_{\overline{i}}) < \frac{n+1}{2}$), $ P(a^{'}_i \cup a^{'}_{\overline{i}}) =\frac{P(a_i)}{P(t)} \times P(t_{\overline{i}}) \times P(t_i)= P(a_i)\times P(t_i)$. Hence, $ P(a^{'}_i \cup a^{'}_{\overline{i}}) \le P(a_i) $.
	
	\item \label{case2.2} If $ Gu(t_{\overline{i}}) $ should vote when either $ Gu(t_i) $ votes for T or F (i.e., $w(a_i)-w(t_{\overline{i}}) < \frac{n+1}{2}$ and $w(a_i)-w(t_i) \ge \frac{n+1}{2}$), $ P(a^{'}_{\overline{i}}) =\frac{P(a_i)}{P(t)} \times P(t_{\overline{i}})= P(a_i)$. Hence, $ P(a^{'}_{\overline{i}}) = P(a_i) $. Clearly, $ P(a^{'}_i) = 0 $.
	
	\item \label{case2.3} If  $ Gu(t_i) $ should vote when either $ Gu(t_{\overline{i}}) $ votes for T or F (i.e., $w(a_i)-w(t_{\overline{i}}) \ge \frac{n+1}{2}$ and $w(a_i)-w(t_i) < \frac{n+1}{2}$), $ P(a^{'}_{\overline{i}}) =\frac{P(a_i)}{P(t)} \times P(t_i)$. Clearly, $ P(a^{'}_{\overline{i}}) = 0 $.
	
	\item\label{case2.4} If at least one of $ Gu(t_i) $ and $ Gu(t_{\overline{i}}) $ should vote for T (i.e., $w(a_i)-w(t_i) < \frac{n+1}{2}$ and $w(a_i)-w(t_{\overline{i}}) < \frac{n+1}{2}$), $ P(a^{'}_i \cup a^{'}_{\overline{i}}) =\frac{P(a_i)}{P(t)} \times (P(t_{\overline{i}}) + (1-P(t_{\overline{i}})) \times P(t_i))$. So, $ P(a^{'}_i \cup a^{'}_{\overline{i}}) \ge P(a_i) $.
	
\end{enumerate}
%\end{enumerate}

% We can go in the opposite direction and reverse the result of each case for $Split$.

These cases show us this important fact that it would be generally impossible to predict (except in some special examples) whether an action has as a positive impact on $ P_{H,\vec{p}}(T) $ or not.

\begin{obs}\label{obs1}
	
	
	If partitioning a tree $ t $ increases $ P_{H,\vec{p}}(T)  $, the result of Case\ref{case2.4} and/or \ref{case2.2}, which have positive impact on a subset $A^{'} \subseteq A$ dominates the result of Case\ref{case2.1}, which has negative impact on $A\setminus A^{'}$.
	
	
\end{obs}

Observation~\ref{obs1} implies that the delegations can sometimes lead to a situation where, some gurus get \textit{surplus power} and some votes assigned to them are left unused to increase the chance of having T as a winner. In other words, partitioning $ t $ into two trees $t_{\overline{i}}, t_i $ leads to $\sum_{i=1}^{|A|} P(a_i) \le \sum_{i=1}^{|A|} P^{'}(a_i)$, i.e., $ P_{H,\vec{p}}(T) \le P_{H^{'}, \vec{p}}(T)$. %More formally, the guru $ Gu(t) $ has a surplus power if a portion of her power has the same positive result as all of her power have \HG{I don't understand this sentence.}.



\begin{exmp}
	Consider the same SN as the one aforementioned for Example\ref{ex1}. In Fig.\ref{unused}, two voters 4 and 5 delegate to 3. So, voter 2 has not enough power to support T. However, if voter 4 votes directly, voter 2 could be helpful in discovering the ground truth (see Fig.\ref{used}). 
	
	\begin{figure}[htbp]
		
		\centering
		
		
		\subfloat[$P_{H,\vec{p}}(T) = 70\%$]{\label{unused}\includegraphics[height=2.5cm,width=4cm]{figures/unused.png}} \hspace{2cm}
		\subfloat[ $P_{H^{'}, \vec{p}}(T) = 79$\%]{\label{used}\includegraphics[height=2.5cm,width=4cm]{figures/used.png}}
		\caption{}
		
		%\label{fig:1}
	\end{figure}
	
	
\end{exmp}


%\HG{If you think this is important, make it a definition, with a definition environment.} A tree $ t_i $ is called an \textit{active} tree if there exists at least a subset $ a_i \in A $ in which $ Gu(t_i) $ should vote for T \HG{what does this mean? I would guess that it means that their exists $ a_i \in A $ such that $a_i\setminus\{t_i\} \notin A$ but it is unclear from your sentence.}. Otherwise, $ t_i $ will be called \textit{inactive} tree. For example, in Fig.\ref{unused}, the tree that only contains voter 2, is denoted as $ t_2 $, is inactive. By changing the delegations and having new delegation graph (see Fig.\ref{used}), we activate $ t_2$.

%\begin{lemma}\label{lemactive}
%	Consider inactive tree $ t_j. $ Performing $ Split $ (or $ReDelegate$) on a tree $t \in \Forest \setminus \left\lbrace t \right\rbrace $ that activates $ t_j $, increases $ P_{H,\vec{p}}(T)$.
%\end{lemma}
%
%\begin{proof}
%	It is obvious that the inactive tree $ t_j $ exists iff there is a tree $t \in \Forest \setminus \left\lbrace t_j \right\rbrace $ with $ w(t) \ge \dfrac{n+1}{2} $ \HG{This is false. Consider 7 voters, 3 trees of size 2 and one singleton. Then the singleton is an inactive tree... Moreover the lemma is clearly false.. Consider a tree of $n-1$ voter where the guru votes for $T$ with probability 1 all other voters having probability 0, and a singleton. It is easy to activate the singleton while highly decreasing the prob of electing T.}. So, we can perform $ Split(t)$ (or $ReDelegate$) in a way that makes $ t_j $ active. By following Case\ref{case2.4}, where $ t_j^{'}=t_j^{'} \cup t_j $ and $t_j^{'} \in \Forest_t$, we conclude that activating $ t_j $ makes T the outcome of election more likely.
%\end{proof}

\section{Greedy Algorithm}
In the following, we will present an iterative greedy approach, denoted by $ k $-GAO (where GAO stands for Greedy Algorithm for $ k $-ODP), in which the outcome of election will be progressively adjusted towards an optimal solution. In each iteration, possible actions (performing $ Join $, $Split$ and $ ReDelegate $ on $ \Forest $) and their impacts on discovering the ground truth are determined. In particular, in each iteration, this approach checks weather joining two different trees if possible, say $ t_i $ and $ t_j $, is beneficial and has positive impact on the outcome (takes $ O(|A|n^{2}) $ time for all pairs $ (t_i, t_j) $ \HG{This looks like an exponential complexity, you should analyse what is the worst value for $|A|$. Is there a way to compute $P(T)$ which is more tractable?}). It specifies if a tree $ t $ has a surplus power. Also, it checks if re-delegations of voters can improve $ P_{H_i, \vec{p}}(T) $. Then, the action with maximum impact in the current iteration is selected. In particular, for each tree $ t $, the possible actions (joining to other possible trees, partitioning into two possible trees and re-delegating) and their impacts on discovering T are specified, which takes $ O(|A|n^{2}) $ times for all trees. The action that has the highest impact on increasing the probability of T is performed. The algorithm is executed $ k $ times, so the total running time is $(k|A|n^{2})$ (in the worst case). It is worth noting that splitting a tree $ t $ into two trees $ (t^{'}_i, t^{'}_j) $ and joining tree $ t^{'}_j$ to another tree is counted as one action (i.e., $ ReDelegate $).

\begin{algorithm}[H]
	\caption{ $k$-GAO }
	\label{Forward}
	\hspace*{\algorithmicindent} \textbf{Input:} $G$, $T$ (the ground truth) and $F$, $H = (V, E) \in \Delta(G)$, $\vec{p}$ and $k$.\\
	\hspace*{\algorithmicindent} \textbf{Output:} $H^{'} = (V, E^{'})\in \Delta(G)$ s.t. $|E^{'}\setminus E|\le k$. 
	\begin{algorithmic}[1]\baselineskip=14pt\relax
		
		\FOR {$ z=1...k$}
		\FOR {every $ t\in S $ }
		
		\STATE Join $ t$ to possible trees, and calculate their impacts on $ P_{H_i, \vec{p}}(T) $;\tcp{$ Join $}
		\STATE Split $ t $ into all two possible trees $ t^{'}_i $ and $ t^{'}_j $, calculate their impacts on $ P_{H_i, \vec{p}}(T) $;  \label{split} \tcp{$Split$}
		
		
		\tcp{Now the effect of each $ t^{'}_j $ on $ P_{H_i, \vec{p}}(T) $ from line\ref{split} is computed}
		\FOR {every $ t^{'}_j $} 
		
		\STATE Join $ t^{'}_j $ to possible trees, and calculate their impacts on $ P_{H_i, \vec{p}}(T) $; \tcp{$ReDelegate$}
		
		\ENDFOR
		\STATE Select the action with the highest impact.
		\ENDFOR
		
		
		
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

%\begin{obs}
%	
%	$k$-GAO converges to an optimal solution.
%	
%	\begin{proof}
%		In each iteration, since we select the action that has positive affect on $ P_{H^{'}, \vec{p}}(T) $, $k$-GAO always takes a positive step toward an optimal solution.
%	\end{proof}
%	
%\end{obs}


Since at each iteration we only do an action if it strictly increases $P_{H,\vec{p}}(T)$, there is no cycle after performing $k$-GAO. $k$-GAO terminates because $k$ is finite.

\begin{remark}
	$k$-GAO is a $ 1/2 $ approximation for $k$-ODP, when $P_{H,\vec{p}}(T) \ge 50\%$.
	%\HG{Ok but any reasonable algorithm is. Maybe this can be a remark which can come much sooner.}.
\end{remark}

It is worth noting that $k$-GAO may converge to a local optimum. 

\begin{exmp}\label{exmplocal}
	Consider the same SN as Example\ref{local} and the delegation graph that every voter votes directly (see Fig.\ref{local}). In the first iteration, since no action can improve $ P_{H,\vec{p}}(T) $, $k$-GAO gets traped in this local optimum. However, the global optimal solution happens when voter 2 and 3 delegates to voter 4 and 5, respectively (see Fig.\ref{global}).
\end{exmp}


\begin{figure}[htbp]
	
	\centering
	
	\subfloat[$P_{H,\vec{p}}(T) = 98.11\%$]{\label{local}\includegraphics[height=2.5cm,width=4cm]{figures/dg21.png}} \hspace{2cm}
	\subfloat[ $P_{H^{'}, \vec{p}}(T) = 99.75\%$]{\label{global}\includegraphics[height=2.5cm,width=4cm]{figures/global.png}}
	\caption{}
	
	
	%\label{fig:1}
\end{figure}

\begin{theorem}
	$k$-GAO is a $p^{k-1}_{min}$ approximation for $k$-ODP, where $ p_{min}=\min_i \vec{p}[i] $.
\end{theorem}
\begin{proof}
	Let $H^{*}$ and $H^{'}$ be the optimal solution and the outcome of $k$-GAO, respectively. Let $ H_i $ and $P_{H_i,\vec{p}}(T)$ be the delegation graph and the probability of selecting T in iteration $ i $, respectively ( i.e., the action $i$, which is either partitioning or joining or the combination of them). 
	
	Give budget $ k $, we first show that the optimal solution $ P_{H^{*},\vec{p}}(T) $ can be bounded with respect to budget $ k $ and $ P_{H,\vec{p}}(T) $. Based on the cases we mentioned before, in $ i $th iteration, for every $ a_j \in A$, after performing one of the actions $ Join $, $Split$ and $ ReDelegate $, $ P^{'}(a_j)=\dfrac{P(a_j)}{p_{min}} $, which is the maximum amount $ P^{'}(a_j) $ can have. So, the optimal solution in iteration $ i $ is $ P_{H^{*}_{i},\vec{p}}(T) \le \frac{P_{H_{i-1},\vec{p}}(T)}{p^{i-1}_{min}}$. Except for the iterations that the optimal solution may decreased (like example~\ref{exmplocal}). In the best case, this happens only at one of the iterations. So, $P_{H^{*},\vec{p}}(T) \le \frac{P_{H,\vec{p}}(T)}{p^{k-1}_{min}}$.
	
	Also, in each iteration, $k$-GAO always selects an action that increases $P_{H_i,\vec{p}}(T)$, unless it gets stuck in a local optimum and does not take into account any action. In the worst case, $k$-GAO leads to a local optimum solution in the first iteration (like example~\ref{exmplocal}). So, $P_{H,\vec{p}}(T) \le P_{H^{'},\vec{p}}(T)$. Hence, $p^{k-1}_{min}\times P_{H^{*},\vec{p}}(T) \le P_{H^{'},\vec{p}}(T)$.
\end{proof}
%\HG{For now, I don't think the theorem is true because I am not convinced by the case analysis you did before but I understand the global idea of the proof you want to build.}

The analysis of the  approximation factor that we gave above is pessimistic. In fact, for each subset $ a_j \subseteq A$, we
bounded its probability by maximum amount in an optimal approach in each iteration, which will not happen for all of the subsets of $A$.


Since ODP is inapproximable problem, we consider a simplified version of ODP in that $ G $ is an undirected graph. 

%Each disjoint set $ d_i \in D$ is rooted at a guru Let us first show that the probability of selecting the grand truth depends on two Activating a disjoint set means that the disjoint set can influence on the probability of the ground truth. In figure~\ref{label}, voters 4 and 5 delegate to voter 3 and voter 2 has no effect on the selecting the ground truth. If voter, say 4, votes directly or re-delegate to voter 2, voter 2 can play in electing the ground truth.


==> contribution/k-odp.tex <==
\section{$k$-ODP}
This section is devoted to another version of ODP, where we are given a delegation graph as input and we are allowed to change at most $k$ delegations to maximize the probability of the ground truth being selected. We term this problem $k$-ODP for Optimal $k$-Delegation Problem. It can be seen as a re-optimization variant of ODP where the parameter $k$ represents a budget parameter modeling the extent to which we are able to change an initial delegation graph. $k$-ODP is formally defined in the following way:\\

\noindent\fbox{\parbox{12.7cm}{
		\textbf{$k$-ODP} (Optimal $ k $-Delegation Problem)\\
		\emph{Input}:\ A social network $G$, two alternatives $T$ (the ground truth) and $F$, a delegation graph $H = (V, E) \in \Delta(G)$, a vector of confidence levels $\vec{p}$ and a budget $k$. \\
		\emph{Feasible Solution}: A delegation graph $H^{'} = (V, E^{'})\in \Delta(G)$ s.t. $|E^{'} \setminus E|\le k$. \\
		\emph{Measure}: $P_{H^{'}, \vec{p}}(T)$ to maximize.
}}\\

One can show that $ K $-ODP is not approximable within a factor of $ \alpha \le 1 $ as ODP. The technique for proving the hardness of $k$-ODP that we provide in the following is almost the same as the reduction described above.

\begin{theorem}\label{KODPth}
	There is no polynomial time algorithm for $ K $-ODP that achieves an approximation guarantee of $\alpha \le 1$, assuming $ P\neq NP $.
	
	\begin{proof}
	
	
	    As Theorem~\ref{ODPth}, we have the reduction from an instance $ I $ of the minimum set cover problem, consisting $ U $ and $ S $, to an instance $ I^{'} $ of $ k$-ODP, consisting a graph $ G $, delegation graph $ H $, vector $\vec{p}$ and a budget $ k $, as follows. In this reduction, we create the same graph $ G $ as Fig.~\ref{dirconsn}. For each $ i \in U $, let $ v_{i1}, v_{i2}, ..., v_{im^{2}} , v_{i(m^{2}+1)}, ..., v_{i(2m^{2})}$ be the nodes in $ V $ such that for every $ j \in [2m^{2}-1] $, there is an directed edge $(v_{ij+1}, v_{ij})$. Also, for each $ i \in [n] $ and $ j \in [m^{2}-1] $ there is a directed edge from $ v_{im^{2}+j}$ to $ v_{im^{2}+j+1}$. For every $i \in [n]$, each voter $v_{i1}$ and $v_{i2m^{2}}$ has a confidence level $ 0 $. Each voter $v_{ij}$ has a confidence level $p_{ij} < 1$, where $j\ne 1, 2m^{2}$. For each $ S_i \in S$, let $ v_{S_i}$ be a node in $ G $, each with confidence level $0.5 \%$. For every $ i\in [n]  $ and $ j \in [m] $, there is an directed edge $\left\lbrace  v_{i,1}, v_{S_j} \right\rbrace $ if $ i \in S_j $. %For every $ i \in [n-1] $, an directed edge $\left\lbrace v_{i, m^{2}+1}, v_{i+1, m^{2}+1}\right\rbrace $ is drawn.
		
		Consider the delegation graph $ H \in \Delta(G)$ as follows (see Fig.~\ref{deldirconsn}). For each $ i \in [n] $ and $ j \in [m^{2}]$, voter $ v_{ij} $ delegates to $ v_{i(j-1)} $. For each $ i \in [n] $ and $ j \in [m^{2}-1] $, voter $ v_{im^{2}+j}$ delegates to voter $ v_{im^{2}+j+1}$. Voters $v_{S_1}, v_{S_2}, ..., v_{S_m}$ vote directly. We define a budget $\bar{k}=n$. Since $v_{12m^{2}}, v_{22m^{2}}, ..., v_{n2m^{2}}$ with the total weight $ nm^{2}$ vote for the alternative F, budget $ n $ is required for which, for every $ i \in [n] $, each voter $ v_{i1} $ delegates to one of the feasible voters $ v_{S_j}, v_{S_j}, ..., v_{S_m} $ in order to have T as the winner. Hence, in the same way as we proved in Theorem \ref{ODPth}, we can show that there is no polynomial time algorithm that deals with $ K$-ODP and achieves an approximation guarantee of $\alpha \le 1$, unless $ P=NP $. 
		





\begin{figure}
\centering
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw = black,
            thick,
            fill = white,
            minimum size = 4mm}
        }
\tikzset{edge/.style = {->,> = latex'}}
% vertices

\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs1) at  (-1,0) {$v_{S_1}$};
\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs2) at  (1,0) {$v_{S_2}$};
\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs3) at  (3,0) {$v_{S_m}$};

\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v11) at  (-1.4,-2) {$v_{11}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v12) at (1,-2) {$v_{12}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v1n) at (3.4,-2) {$v_{1n}$};

\node[vertex][minimum size=1.5cm] (v21) at  (-1.4,-4) {$v_{21}$};
\node[vertex][minimum size=1.5cm] (v22) at (1,-4) {$v_{22}$};
\node[vertex][minimum size=1.5cm] (v2n) at (3.4,-4) {$v_{2n}$};

\node[vertex][minimum size=1.5cm] (v1m2) at  (-1.4,-6) {$v_{1m^{2}}$};
\node[vertex][minimum size=1.5cm] (v2m2) at (1,-6) {$v_{2m^{2}}$};
\node[vertex][minimum size=1.5cm] (vnm2) at (3.4,-6) {$v_{nm^{2}}$};

\node[vertex][minimum size=1.5cm] (v1m2+1) at  (-1.4,-8) {$v_{1m^{2}+1}$};
\node[vertex][minimum size=1.5cm] (v2m2+1) at (1,-8) {$v_{2m^{2}+1}$};
\node[vertex][minimum size=1.5cm] (vnm2+1) at (3.4,-8) {$v_{nm^{2}+1}$};

\node[vertex][minimum size=1.5cm] (v1m2+2) at  (-1.4,-10) {$v_{1m^{2}+2}$};
\node[vertex][minimum size=1.5cm] (v2m2+2) at (1,-10) {$v_{2m^{2}+2}$};
\node[vertex][minimum size=1.5cm] (vnm2+2) at (3.4,-10) {$v_{nm^{2}+2}$};

\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v12m2) at  (-1.4,-12) {$v_{12m^{2}}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v22m2) at (1,-12) {$v_{22m^{2}}$};
\node[vertex][minimum size=1.5cm, label=right:{0\%}] (vn2m2) at (3.4,-12) {$v_{n2m^{2}}$};


%edges
\draw[edge] (v11) to (vs1);
\draw[edge] (v11) to (vs3);
\draw[edge] (v12) to (vs1);
\draw[edge] (v12) to (vs2);
\draw[edge] (v1n) to (vs1);
\draw[edge] (v1n) to (vs3);


\draw[edge] (v21) to (v11);
\draw[edge] (v22) to (v12);
\draw[edge] (v2n) to (v1n);

\draw[edge] (v1m2+1) to (v1m2);
\draw[edge] (v2m2+1) to (v2m2);
\draw[edge] (vnm2+1) to (vnm2);

\draw[edge] (v1m2+1) to (v1m2+2);
\draw[edge] (v2m2+1) to (v2m2+2);
\draw[edge] (vnm2+1) to (vnm2+2);

\draw[edge] (v1m2+2) to (v1m2+1);
\draw[edge] (v2m2+2) to (v2m2+1);
\draw[edge] (vnm2+2) to (vnm2+1);




%paths
\path (vs2) to node {\dots} (vs3);
%\path (vs2) -- (vs3) node [ midway, sloped] {$\dots$};
\path (v12) to node {\dots} (v1n);
\path (v22) to node {\dots} (v2n);
\path (v2m2) to node {\dots} (vnm2);


\path (v1m2) -- (v21) node [ midway, sloped] {$\dots$};
\path (v2m2) -- (v22) node [ midway, sloped] {$\dots$};
\path (vnm2) -- (v2n) node [ midway, sloped] {$\dots$};

\path (vnm2) -- (v2n) node [ midway, sloped] {$\dots$};
\path (v12m2) -- (v1m2+2) node [ midway, sloped] {$\dots$};
\path (v22m2) -- (v2m2+2) node [ midway, sloped] {$\dots$};
\path (vn2m2) -- (vnm2+2) node [ midway, sloped] {$\dots$};
%\path (n6) -- (n7) node [red, font=\Huge, midway, sloped] {$\dots$};
%\path (vn1) to node {\dots} (v21);
%\path (vn1) -- node[auto=false]{\ldots} (v21);

\end{tikzpicture}%

\caption{The SN}\label{dirconsn}

\end{figure}

\begin{figure}

\centering
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw = black,
            thick,
            fill = white,
            minimum size = 4mm}
        }
\tikzset{edge/.style = {->,> = latex'}}
% vertices

\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs1) at  (-1,0) {$v_{S_1}$};
\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs2) at  (1,0) {$v_{S_2}$};
\node[vertex][minimum size=1.5cm, label=above:{50\%}] (vs3) at  (3,0) {$v_{S_m}$};

\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v11) at  (-1.4,-2) {$v_{11}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v12) at (1,-2) {$v_{12}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v1n) at (3.4,-2) {$v_{1n}$};

\node[vertex][minimum size=1.5cm] (v21) at  (-1.4,-4) {$v_{21}$};
\node[vertex][minimum size=1.5cm] (v22) at (1,-4) {$v_{22}$};
\node[vertex][minimum size=1.5cm] (v2n) at (3.4,-4) {$v_{2n}$};

\node[vertex][minimum size=1.5cm] (v1m2) at  (-1.4,-6) {$v_{1m^{2}}$};
\node[vertex][minimum size=1.5cm] (v2m2) at (1,-6) {$v_{2m^{2}}$};
\node[vertex][minimum size=1.5cm] (vnm2) at (3.4,-6) {$v_{nm^{2}}$};

\node[vertex][minimum size=1.5cm] (v1m2+1) at  (-1.4,-8) {$v_{1m^{2}+1}$};
\node[vertex][minimum size=1.5cm] (v2m2+1) at (1,-8) {$v_{2m^{2}+1}$};
\node[vertex][minimum size=1.5cm] (vnm2+1) at (3.4,-8) {$v_{nm^{2}+1}$};

\node[vertex][minimum size=1.5cm] (v1m2+2) at  (-1.4,-10) {$v_{1m^{2}+2}$};
\node[vertex][minimum size=1.5cm] (v2m2+2) at (1,-10) {$v_{2m^{2}+2}$};
\node[vertex][minimum size=1.5cm] (vnm2+2) at (3.4,-10) {$v_{nm^{2}+2}$};

\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v12m2) at  (-1.4,-12) {$v_{12m^{2}}$};
\node[vertex][minimum size=1.5cm, label=left:{0\%}] (v22m2) at (1,-12) {$v_{22m^{2}}$};
\node[vertex][minimum size=1.5cm, label=right:{0\%}] (vn2m2) at (3.4,-12) {$v_{n2m^{2}}$};


%edges

\draw[edge] (v21) to (v11);
\draw[edge] (v22) to (v12);
\draw[edge] (v2n) to (v1n);


\draw[edge] (v1m2+1) to (v1m2+2);
\draw[edge] (v2m2+1) to (v2m2+2);
\draw[edge] (vnm2+1) to (vnm2+2);






%paths
\path (vs2) to node {\dots} (vs3);
%\path (vs2) -- (vs3) node [ midway, sloped] {$\dots$};
\path (v12) to node {\dots} (v1n);
\path (v22) to node {\dots} (v2n);
\path (v2m2) to node {\dots} (vnm2);


\path (v1m2) -- (v21) node [ midway, sloped] {$\dots$};
\path (v2m2) -- (v22) node [ midway, sloped] {$\dots$};
\path (vnm2) -- (v2n) node [ midway, sloped] {$\dots$};

\path (vnm2) -- (v2n) node [ midway, sloped] {$\dots$};
\path (v12m2) -- (v1m2+2) node [ midway, sloped] {$\dots$};
\path (v22m2) -- (v2m2+2) node [ midway, sloped] {$\dots$};
\path (vn2m2) -- (vnm2+2) node [ midway, sloped] {$\dots$};
%\path (n6) -- (n7) node [red, font=\Huge, midway, sloped] {$\dots$};
%\path (vn1) to node {\dots} (v21);
%\path (vn1) -- node[auto=false]{\ldots} (v21);


\end{tikzpicture}
\caption{The delegation graph.}\label{deldirconsn}


\end{figure}  
\end{proof}
\end{theorem}

Theorem~\ref{KODPth} implies that $ k $-ODP is inapproximable even if an optimal set of gurus is known in advance, and it would be hard to find the optimal delegation graph. Let $ Gu(H) $ be the set of all gurus in $ H $. Let $ H^{*} $ be the optimal solution. By following Theorem~\ref{KODPth}, one can show that even the simplified version of $ k$-ODP, denoted by $ k $-ODPG, in which, $ H $ and $Gu(H)$ are given as input where $ H\ne H^{*} $ and $ Gu(H)=Gu(H^{*}) $, and by changing the opinions of at most $ k $ followers, we are asked to find the delegation graph $H^{*}$, is inapproximable within a factor of $\alpha \le 1$. More formally,\\

\noindent\fbox{\parbox{12.7cm}{
		\textbf{$k$-ODPG}\\
		\emph{Input}:\ A social network $G$, two alternatives $T$ (the ground truth) and $F$, a delegation graph $H = (V, E) \in \Delta(G)$, a (optimal) set of gurus $ Gu(H) $, a vector of confidence levels $\vec{p}$ and a budget $k$. \\
		\emph{Feasible Solution}: A delegation graph $H^{'} = (V, E^{'})\in \Delta(G)$ s.t. $|E^{'} \setminus E|\le k$ and $ Gu(H^{'})=Gu(H) $. \\
		\emph{Measure}: $P_{H^{'}, \vec{p}}(T)$ to maximize.
}}\\


Theorem~\ref{KODPth} then implies the following corollary.
\begin{corollary}\label{corODPG}
	$ k $-ODPG is inapproximable within a factor of $\alpha \le 1$.
\end{corollary}

Corollary~\ref{corODPG} shows that the most difficult part of the main research question is how to partition the graph and assign weights to the gurus.

==> contribution/odpu.tex <==
\section{Approximation Algorithm for ODPU}\label{secodpu}
In this section, we investigate ODPU, another variant of ODP where the input is an undirected connected graph instead of a directed one:\\

\noindent\fbox{\parbox{12.7cm}{
		\textbf{ODPU}\\
		\emph{Input}: An undirected connected graph $G$ and an accuracy vector $\vec{p}$.\\
		\emph{Feasible Solution}: A delegation function $d$. \\
		\emph{Measure}: $P_{d, \vec{p}}$ to maximize.
}}\\

Note that, because the graph is undirected and connected, it is possible for all voters to delegate to the same guru. Interestingly, we will see that the simple strategy in which all voters delegate to one of the most ``competent'' voter $v^* \in \text{arg}\max\{p_i|i\in V\}$ leads to a 2-approximation algorithm for the ODPU problem. We call this strategy the \emph{best guru strategy}. 
\begin{theorem}
	The best guru strategy leads to a $ 1/2 $-approximation algorithm for the ODPU problem. 
\end{theorem}

As this result is straightforward when $p_{\max} = \max\{p_i|i\in V\}$ is greater than or equal to $0.5$, we focus on the case where $p_{\max} < 0.5$. In the rest of this section, we show that in this case, the best guru strategy is optimal.



%Before presenting the algorithm, we would like to consider the social networks where people believe that the alternative $ F $ is the correct answer more likely. In these social networks, we suppose that voters' beliefs are less accurate than a random guess. In particular, every voter $ i $ intends to cast a vote for $ T $ with probability $ p_i < 1/2$. We pay special attention to these social networks and show how much accurate delegation mechanisms can be in this case. So, in the following, we aim to bound the optimal solution, where $ p_{max} < 0.5$. We first consider the case where all voters vote directly (i.e., direct democracy). Let $P=2^{V}$. To prove Theorem~\ref{bounddelegation}, we introduce the following notions.
\begin{definition}
	Given a delegation function $d$, a subset $S \subseteq Gu(d)$ is \textit{successful} if $w(S) \ge \lceil n/2 \rceil$, otherwise it is \textit{unsuccessful}. We denote by $\text{Succ}(d)$ (resp. $\text{UnSucc}(d)$), the set of successful (resp. unsuccessful) sets in $Gu(d)$.
\end{definition}
Put another way, a set $S$ of gurus is successful if $T$ is elected when the set of gurus voting correctly is $S$; $S$ is called unsuccessful otherwise.

\begin{comment}
\begin{definition}
	Given a delegation function $d$, let the \emph{truth set} $\mathcal{X}_d$ denote the random variable denoting the set of gurus voting correctly. %By abuse of notation, we will say that the truth set is \textit{successful} if the realization of $X$ is a successful set; it is called \textit{unsuccessful} otherwise.
\end{definition}
\end{comment}

\begin{comment}

Given a delegation graph $H \in \Delta(G)$ and an interval $\left[ w_l, w_m\right]$ for some $ w_l, w_m \in [1..n] $, where $ n $ is the number of voters. Let $ z \in [1..q] $ such that $ q=|Gu(H)| $. Let $S \in \text{Succ}(H)$ and $ S^{'} \in Gu(H) \setminus \text{Succ}(H) $.

\begin{definition}
We say that $ Gu(H)$ over the interval $ \left[ w_l, w_m\right]  $ is \textit{symmetric} if for any successful subset $S$ that votes for T with the probability of $ P(S)=p^{z}(1-p)^{q-z} $, where $w(S) \in \left[ w_l, w_m\right] $ there is an unsuccessful subset $S^{'}$ that votes for F with the probability of $P(S^{'})=p^{z-1}(1-p)^{q-z+11}$, where $w(S^{'}) \in \left[ w_l, w_m\right]$.
\end{definition}
\end{comment}


We will also require the following lemma:
\begin{lemma}\label{lemma:pmax}
	Given a confidence vector $\vec{p}$, let $\vec{p}_{\max}$ be the vector obtained from $\vec{p}$ by raising all its entries to $p_{\max}$, then for any delegation function $d$, $P_{d,\vec{p}}(T) \le P_{d,\vec{p}_{\max}}(T)$.
\end{lemma}
\begin{proof}
	By following the recursive formula~\ref{lbrecursiveformula}, we have
	\begin{align*}
	\quad F(\tau > 0,i) &= p_{g_i} F(\tau - w(i,H),i+1) + (1-p_{g_i})F(\tau,i+1)\\
	&= F(\tau,i+1) + p_{g_i} (F(\tau - w(i,H),i+1) - F(\tau,i+1))
	\end{align*}
	The result then follows from the fact that $F(\tau',j) - F(\tau,j)\ge 0$, when $\tau'\le \tau$.
\end{proof}



\begin{comment}


\HG{To be removed after.}
\begin{lemma}\label{bound}

$P_{H^D,\vec{p}}(T) \le p_{max}$, where $p_{max} < 1/2$ and $ H^D $ is a delegation graph in which every voter votes directly.

\begin{proof}
We make a proof by induction on the number of voters. Using Lemma~\ref{lemma:pmax}, we will suppose that all voters vote with the probability of $ p=p_{max}$. Let $H^D_n$ denote the delegation graph $H^D$ defined on $n$ voters. If $n=1$, the result is straightforward. Let us assume the result true for an odd number of voters $n \ge 1 $. Put another way, denoting by $z_n(i)$ the value $\binom{n}{i} p^{i}(1-p)^{n-i}$, we assume that, 
$$P_{H^{D}_n,\vec{p}}(T)=\sum_{S \in \text{Succ}(H^D_n)} P[\mathcal{X}_{H^D_n} = S] = \sum_{i=\lceil n/2 \rceil}^{n} z_n(i)\le p.$$ 

We want to prove that $P_{H^{D}_{n+2},\vec{p}}(T) \le p$. Stated differently, we want to show that the result remains true if we add two new voters $ v_{n+1} $ and $ v_{n+2} $ to the election such that $p_{v_{n+1}} = p_{v_{n+2}} = p$. Let us consider $S \in V(H^{D}_{n+2})$ and $W = S\cap V(H^{D}_{n})$. Then, we make the following simple observations: 
\begin{itemize}
\item if $|W| < \lfloor n/2\rfloor$, then $S\notin \text{Succ}(H^D_{n+2})$;
\item if $|W| > \lceil n/2\rceil + 1$, then $S\in \text{Succ}(H^D_{n+2})$;
\item if $|W| = \lceil n/2\rceil$, then $S\in \text{Succ}(H^D_{n+2})$ iff $S\cap\{v_{n+1},v_{n+2}\} \neq \emptyset$. 
\item if $|W| = \lfloor n/2\rfloor$, then $S\in \text{Succ}(H^D_{n+2})$ iff $\{v_{n+1},v_{n+2}\} \subseteq S$. 
\end{itemize}
From these observations, we obtain that $P_{H^{D}_{n+2},\vec{p}}(T)$ can be rewritten as:
\begin{align*}
P_{H^{D}_{n+2},\vec{p}}(T) =& \big(\sum_{i=\lceil n/2 \rceil + 1}^{n} z_n(i)\big)
+ z_n(\lceil n/2 \rceil) (p^2+2p(1-p)) 
+ z_n(\lfloor n/2 \rfloor)p^2 .
\end{align*}
And hence:
\begin{align*}
P_{H^{D}_{n+2},\vec{p}}(T) - P_{H^{D}_{n},\vec{p}}(T) =& z_n(\lfloor n/2 \rfloor)p^2 
- z_n(\lceil n/2 \rceil)(1-p)^2 \\
=& {n \choose \lfloor n/2 \rfloor}p^{\lceil n/2 \rceil}(1-p)^{\lceil n/2 \rceil}(2p -1) \le 0
\end{align*}
where we have used the fact that ${n \choose \lfloor n/2 \rfloor} = {n \choose \lceil n/2 \rceil}$ and $p < 0.5$. Consequently, we obtain that $P_{H^{D}_{n+2},\vec{p}}(T) \le  P_{H^{D}_{n},\vec{p}}(T) \le p_{\max}$ which concludes the proof. 


%\begin{equation}\label{eqhypothesis}
%P_{H^{*},\vec{p}}(T)=\sum_{i=\lfloor (n+2)/2\rfloor +1 }^{n+2} \binom{n+2}{i}p^{i}(1-p)^{n+2-i}\le p.
%\end{equation}


%Stated differently, we want to show that $P_{H^{*},\vec{p}}(T)$ is still less than or equal to $p < 1/2$, if we add two new voters $ v_{n+1} $ and $ v_{n+2} $ to the election such that $\max(p_{v_{n+1}}, p_{v_{n+2}})\le p$. Let $ V_n $ be the set of voters when the number of voters is $ n $. Let the truth set $ X_n$ denote the random variable denoting the set of gurus (voters) voting correctly. When we add two new voters, the truth set $ X_{n+2} $ is successful if  its realization set $ x_{n+2} $ is successful, which means that $|x_{n+2}|\ge \lfloor (n+2)/2\rfloor + 1$.  It is worth mentioning that after adding new voters $ v_{n+1} $ and $ v_{n+2} $, the probability of subsets $ V_n $ that have cardinality weights are either less than $ \lfloor n/2\rfloor$ or more than $ \lfloor n/2\rfloor +1$ are not changed. In particular, let $ V^{'}_n$ be the set of all the realization sets with the cardinalites of either less than $ \lfloor n/2\rfloor$ or more than $ \lfloor n/2\rfloor +1$. Obviously, they are remained successful (or unsuccessful) if either $ v_{n+1} $ or $ v_{n+2} $ (or both) cast a vote for T or F. More precisely, let $c \in V^{'}$ with the cardinality of more than $ \lfloor n/2\rfloor +1$, which is a successful realization set. So, the cardinality of $ c $ is at least $ \lfloor n/2\rfloor +3$. Let $ P(c) $ be the probability $ c $ votes for the ground truth. Let $ c^{'}= c \cup \left\lbrace v_{n+1}, v_{n+2}\right\rbrace $. If both voters either vote for T or F,

%$$ P(c^{'})=P(c)\times (p^{2} + 2p(1-p)+(1-p)^{2})= P(c).$$

%In the same way, we can show that if $c \in V^{'}_n$ with the cardinality of less than $ \lfloor n/2\rfloor$, by adding these two new voters, the probability it votes for F is not changed.

%So, the key observation here required for the proof is the following one: by adding these two new voters $ v_{n+1} $ and $ v_{n+2} $, we can only focus on the truth sets $ X_{n} $ that can be changed from successful truth sets to unsuccessful truth sets, and vice versa. Obviously, the unsuccessful truth sets that can turn into successful ones, and vice versa, by adding these two voters are the truth sets with the realization sets of cardinality $ \lfloor n/2\rfloor$ and $ \lfloor n/2\rfloor +1$. Let $ A_n $ and $ B_n $ be the set of all the truth realization sets of cardinality $ \lfloor n/2\rfloor$ and $ \lfloor n/2\rfloor +1$, respectively.

%Consider a truth realization set $ a_i \in A_n$. Before adding the two voters, $ a_i $ is an unsuccessful set, which means that voters in $ a_i $ vote with the probability of $ P(a_i)=p^{\lfloor n/2\rfloor}(1-p)^{\lfloor n/2\rfloor +1}  $ in favor of the alternative F. For every $ i\in [|A_n|] $, let $a^{'}_i=a_i \cup \left\lbrace v_{n+1}, v_{n+2} \right\rbrace $. With respect to $ P(a_i) $, in the following possible value of $ P(a^{'}_i) $ is examined.

%\begin{enumerate}
%	\item If both voters vote for T, $ a^{'}_i$ votes for the ground truth with the probability of 

%	\begin{equation}\label{eqA1}
%	P(a^{'}_i)=P(a_i)\times p^{2}=p^{\lfloor n/2\rfloor +2}(1-p)^{\lfloor n/2\rfloor +1}.
%	\end{equation}

%	\item If either $ v_{n+1} $ or $ v_{n+2}  $ votes for F, $ a^{'}_i$ votes for F with the probability of 

%	\begin{equation}\label{eqA2}
%	P(a^{'}_i)=2 \times P(a_i) p(1-p)=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor +2}.
%	\end{equation}

%	\item If both voters vote for F, $ a^{'}_i$ votes for F with the probability of 

%	\begin{equation}\label{eqA3}
%	P(a^{'}_i)= P(a_i) (1-p)^{2}=p^{\lfloor n/2\rfloor}(1-p)^{\lfloor n/2\rfloor +3}.
%	\end{equation}

%\end{enumerate}

%We suppose $ A^{'}_m $ is the set of all subsets $ a^{'}_i $ that vote for the ground truth with the probability of $ P(a_i)\times p^{2} $.


%Consider a truth realization set $b_j \in B_n$. Before adding these two voters, $ b_j $ is a successful set, which means that voters in $ b_j $ vote for T with the probability of $P(b_j)=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor}$. Let $b^{'}_j=b_j \cup \left\lbrace v_{n+1}, v_{n+2} \right\rbrace $. With respect to $ P(b_j) $, in the following possible value of $ P(b^{'}_j) $ is examined.

%\begin{enumerate}
%	\item If both voters vote for T, $ b^{'}_j$ votes for the ground truth with the probability of 

%	\begin{equation}\label{eqB1}
%	P(b^{'}_j)=P(b_j)\times p^{2}=p^{\lfloor n/2\rfloor +3}(1-p)^{\lfloor n/2\rfloor}.
%	\end{equation}

%	\item If either $ v_{n+1} $ or $ v_{n+2}  $ votes for T, $ a^{'}_i$ votes for T with the probability of 

%	\begin{equation}\label{eqB2}
%	P(a^{'}_i)=2 \times P(b_j) p(1-p)=p^{\lfloor n/2\rfloor +2}(1-p)^{\lfloor n/2\rfloor +1}.
%	\end{equation}

%	\item If both voters vote for F, $ b^{'}_j$ votes for F with the probability of 

%	\begin{equation}\label{eqB3}
%	P(b^{'}_j)=P(b_j)\times (1-p)^{2}=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor +2}. 
%	\end{equation}
%\end{enumerate}

%We suppose $ B^{'}_m $ is the set of all subsets $ b^{'}_j$ that vote for the alternative F with the probability of $ P(b_j)\times (1-p)^{2} $.

%The number of realization sets in their relevant Equations \ref{eqA1}, \ref{eqA2} and \ref{eqA3} are equal to the number of realization sets in their relevant Equations \ref{eqB3}, \ref{eqB2} and \ref{eqB1}, respectively. So, it is enough to show that the sum of Equations \ref{eqA1}, \ref{eqB1} and \ref{eqB2} is less than the sum of Equations \ref{eqA2}, \ref{eqA3} and \ref{eqB3}. Since $ p< 1/2 $, this holds, which implies that if we add new voters $ v_{n+1} $ and $ v_{n+2} $, the probability of wining the ground truth is getting decreased. Therefore, Equation \ref{eqhypothesis} holds and this induction proves the lemma.

\end{proof}

\end{lemma}
\end{comment}

The following theorem shows that the best guru strategy is in fact optimal if $p_{max}<1/2$.
\begin{theorem}\label{bounddelegation}
	If $p_{\max} < 0.5$, then for every delegation function $d$, we have that $P_{d,\vec{p}} \le p_{max}$.
	%$P_{H^{*},\vec{p}}(T) \le p_{max}$, where $p_{max} < 1/2$.
\end{theorem}


	%To prove Theorem~\ref{bounddelegation}, we first introduce the technique we want to use and then prove Lemma~\ref{lmDifAandB} that is required in the proof of Theorem~\ref{bounddelegation}. In particular, we make a proof by induction on the number of gurus in $ Gu(d)$ and show that for any mechanism as long as the number of gurus are increased, the difference between the probability that it selects F and the probability it selects T is greater than or equal to $1-2p$, which concludes Theorem~\ref{bounddelegation}.
	Let $I = (G,\vec{p})$ be an instance of ODP such that $p_{max} < 0.5$ and $d$ be a delegation function defined on this instance. 
    Note that by using Lemma~\ref{lemma:pmax}, we can in fact assume that all voters have accuracy $p=p_{max}$. 
    To prove that $P_{d,\vec{p}} \le p_{max}$, we make a proof by induction on the number of gurus in $Gu(d)$. 
    More precisely, let us order the gurus in $Gu(d)$ such that $Gu(d) = \{g_1,\ldots,g_{|Gu(d)|}\}$. 
    We let $I_i = (G_i,\vec{p_i})$ and $d_i$ denote the restriction of instance $I$ and delegation function $d$ to the $i$ first gurus in $Gu(d)$ and people who delegated to them. 
	We then show by induction that for increasing values of $i$, we have that $P_{d_i,\vec{p_i}} \le p_{max}$ in instance $I_i$.
	
	In our induction, in order to have an odd number of voters at each step, we order the gurus in $Gu(d)$ while respecting the following constraints.  
	The first guru $g_1$ is selected such that $w(g_1)$ is odd. 
	Then, if for $i\in \{1,\ldots,|Gu(d)|\}$, we have that $\sum_{j = 1}^i w(g_j)$ is odd, then either $w(g_{i+1})$ is even, or   $w(g_{i+1})$ and $w(g_{i+2})$ are both odd. 
	In the first case, the induction will move from instance $I_i$ to instance $I_{i+1}$. 
	In the second case, the induction will move from instance $I_i$ to instance $I_{i+2}$.  

	%At the first step, tree $t_1$ includes an odd numbers of voters. At the other steps, we add either two trees $t_i$ and $t_{i+1}$ with odd number of voters each (case 1), or one tree $t_i$ with even number of voters (case 2). The latter case will be proved, and the former one can be proved in the same way. %In the case where only one tree with an even number of voters is remained to add, the lemma holds again (we will see in last part of the proof). 
	
		
	The fact that $P_{d_i,\vec{p_i}} \le p$ for $i=1$ is straightforward. 
	Let us assume the result true for $ i \ge 1$, such that  $n_i := \sum_{j = 1}^i w(g_j)$ is odd. 
	Put another way, we assume that,
	$$P_{d_i,\vec{p_i}} = \sum_{S \in \text{Succ}(d_i)} P[\mathcal{X}_{d_i} = S] \le p.$$
%	In Theorem~\ref{bounddelegation}, if $i=1$, the result is straightforward. Let us assume the result is true for $ i \ge 1$ gurus, where the number of voters is $ n_i $ and odd. Put another way, we assume that,
%	$$P_{H_i,\vec{p}}(T)=\sum_{S \in \text{Succ}(H_i)} P[\mathcal{X}_{H_i} = S] \le p.$$
	
	Let us assume that we are in the case where $w(g_{i+1})$ is even. 
	We then show that $P_{d_{i+1},\vec{p_{i+1}}} \le p$. 
	Let us consider $S \subseteq Gu(d_{i+1})$ and $W = S \cap Gu(d_{i})$. 
    We make the following observations:
		
%	We want to prove that $P_{H_{i+1},\vec{p}}(T) \le p$ in Theorem~\ref{bounddelegation}. Stated differently, we want to show that the result remains true if we add a new guru $ t_{i+1} $ with even cardinality to the election such that $p_{t_{i+1}} = p$. Let us consider $S \in Gu(H_{i+1})$ and $W = S\cap Gu(H_{i})$. Let $ w_{i+1}=w(t_{i+1})$. Let us supposed that the new guru can turn a successful set in $Gu(H_{i})$ to an unsuccessful one in $Gu(H_{i+1})$ and vice versa (otherwise it is clear that Theorem~\ref{bounddelegation} holds). Then, we make the following simple observations: 
	\begin{itemize}
		\item if $w(W) \le \lfloor n_i/2 \rfloor - w(g_{i+1})/2$, then $S\notin \text{Succ}(d_{i+1})$;
		
		\item if $w(W) \ge \lceil n_i/2\rceil + w(g_{i+1})/2$, then $S\in \text{Succ}(d_{i+1})$;
			
		\item if $\lceil n_i/2\rceil \le w(W) < \lceil n_i/2\rceil + w(g_{i+1})/2$, then $S\in \text{Succ}(d_{i+1})$ iff $g_{i+1} \in S$. Let $ B $ be the set of all the corresponding subsets $ W $.
			
		\item if $ \lfloor n_i/2 \rfloor - w(g_{i+1})/2 < w(W) \le \lfloor n_i/2\rfloor $, then $S\in \text{Succ}(d_{i+1})$ iff $g_{i+1} \in S$. Let $ A$ be the set of all the corresponding subsets $ W $.
	\end{itemize}
	
	From these observations, we obtain: %that $P_{H_{i+1},\vec{p}}(T)$ can be rewritten as:
	\begin{align*}
		P_{d_{i+1},\vec{p}}(T) =& \sum_{S' \in \text{Succ}(d_i)\setminus B} P[\mathcal{X}_{d_i} = S']+ p(\sum_{W \in A} P(W) + \sum_{W \in B} P(W))\\
		P_{d_{i+1},\vec{p}}(F) =& \sum_{S' \in \text{UnSucc}(d_i)\setminus A} P[\mathcal{X}_{d_i} = S'] + (1-p)(\sum_{W \in B}  P(W)+ \sum_{W \in A} P(W))
      \end{align*}

In the following, for simplicity, we let $b=\sum_{S' \in \text{Succ}(d_i)\setminus B} P[\mathcal{X}_{d_i} = S']$ and $a=\sum_{S' \in \text{UnSucc}(d_i)\setminus A} P[\mathcal{X}_{d_i} = S']$.

Now, we can prove Theorem~\ref{bounddelegation}.


\begin{proof}[Proof of Theorem~\ref{bounddelegation}]

Assume by contradiction that there exists a delegation function $d_{i+1}$ such that 
\begin{align}\label{eqSumEpsilonT}
    P_{d_{i+1},\vec{p}}(T) = b + p(\sum_{W \in A} P(W) + \sum_{W \in B} P(W))=p+\epsilon.
\end{align}


where $\epsilon > 0$. It implies that 
\begin{align*}
   \sum_{W \in A} P(W) + \sum_{W \in B} P(W)=(p+\epsilon-b)/p.
\end{align*}

So, we have

\begin{equation}\label{eqSumEpsilonF}
   \begin{split}
       P_{d_{i+1},\vec{p}}(F) =& a+ (1-p)(\sum_{W \in B}  P(W)+\sum_{W \in A}P(W))\\ =& a+(1-p)(p+\epsilon-b)/p=a+(p+\epsilon-b)/p-p-\epsilon+b
   \end{split}
\end{equation}

By Equations~\ref{eqSumEpsilonT} and \ref{eqSumEpsilonF},

\begin{align*}
    P_{d_{i+1},\vec{p}}(F)+P_{d_{i+1},\vec{p}}(T)\\=&a+(p+\epsilon-b)/p-p-\epsilon+b+p+\epsilon\\=& a+(p+\epsilon-b)/p+b \\=& a+1+\epsilon/p-b/p+b \\ \ge& 1+a+\epsilon/p \quad \text{ as  $b\le p$ using induction hypothesis}\\ \ge & 1+\epsilon/p \quad \text{ as $a\ge 0$}
\end{align*}
, which contradicts the fact that 
$$P_{d_{i+1},\vec{p}}(F)+P_{d_{i+1},\vec{p}}(T)=1.$$

Hence $\epsilon=0$ and

$$P_{d_{i+1},\vec{p}}(T)\le p$$
, and the theorem is proven in this case.

\begin{comment}


For the case where two new gurus $g_{i+1}$ and $g_{i+2}$ are added, one can prove that Theorem~\ref{bounddelegation} holds. In particular, let us consider $S \in Gu(d_{i+2})$ and $W = S\cap Gu(d_i)$ and $w_{i+1}=w(g_{i+1})+w(g_{i+2})$. Then, we make the following simple observations: 
    \begin{itemize}
		\item if $\lceil n_i/2\rceil \le w(W) < \lceil n_i/2\rceil + w_{i+1}/2$, then $S\in \text{Succ}(d_{i+2})$ iff $S\cap\{g_{i+1}, g_{i+2}\} \neq \emptyset$. Let $ B_i $ be the set of all the relevant subsets $ W $.
			
		\item if $ \lfloor n_i/2\rfloor \le w(W) < \lfloor n_i/2\rfloor + w_{i+1}/2$, then $S\in \text{Succ}(d_{i+1})$ iff $\{g_{i+1}, g_{i+2}\} \subseteq S$. Let $ A_i $ be the set of all the relevant subsets $ W $.
	\end{itemize}
	
So, we have 

\begin{align*}
    P_{d_{i+2},\vec{p}}(T) =& b + \sum_{W \in B_{i}}  P(W)(p^{2}+ 2p(1-p)) + \sum_{W \in A_{i}} P(W)p^{2}.
\end{align*}

And,

\begin{align*}
    P_{d_{i+2},\vec{p}}(F) =& a+(1-p)^{2}\sum_{W \in B_{i}} P(W) + ((1-p)^{2}+2p(1-p))\sum_{W \in A_{i}} P(W).
\end{align*}

Let us again assume by contradiction that there exists a delegation function $d_{i+1}$ such that

\begin{align*}
    P_{d_{i+2},\vec{p}}(T) =& b + (2p-p^{2})\sum_{W \in B}P(W) + p^{2}\sum_{W \in A} P(W)=p+\epsilon
\end{align*}

where $\epsilon>0$. By induction assumption, $b=\le P_{d_i,\vec{p}}(T) \le p$. Let $\sum_{W \in B} P(W)=x \le p$. Thus,

$$(2p-p^{2})\sum_{W \in B} P(W) + p^{2}\sum_{W \in A} P(W)= \epsilon +x \quad \text{, where  $0 \le x \le p$}$$

Consider the case where $\sum_{W \in B} P(W)=x=0$. Since $|A|=|B|$, $\sum_{W \in A} P(W)=0$, which means that

$$(2p-p^{2})\sum_{W \in B}P(W) + p^{2}\sum_{W \in A} P(W)=0=x+\epsilon$$

, which is a contradiction as $\epsilon >0$. So, we suppose that $$(2p-p^{2})\sum_{W \in B} P(W) + p^{2}\sum_{W \in A_{i}} P(W)= p+\epsilon -\gamma \quad \text{ where  $ \gamma <b$}$$

So, $P_{d_{i+2},\vec{p}}(F)$ can be rewritten as,

\begin{equation}\label{eqCase2F}
\begin{split}
P_{d_{i+2},\vec{p}}(F) =& a+\sum_{W \in B} P(W)+\sum_{W \in A} P(W) \\-& ((2p-p^{2})\sum_{W \in B}P(W) + p^2\sum_{W \in A} P(W))\\=& a+\sum_{W \in B} P(W)+\sum_{W \in A} P(W) -(p+\epsilon-\gamma).
\end{split}
\end{equation}

So, we have

\begin{align*}
    P_{d_{i+2},\vec{p}}(F)+P_{d_{i+2},\vec{p}}(T)\\=& a+\sum_{W \in B} P(W)+\sum_{W \in A} P(W) -(p+\epsilon-\gamma)+p+\epsilon \\=& a+\sum_{W \in B} P(W)+\sum_{W \in A} P(W)+\gamma \\ & \ge 1-p+\sum_{W \in B}P(W)+\gamma\quad \text{ as $a+\sum_{W \in A} P(W)=P_{d_i,\vec{p}}(T) \ge 1-p$}
\end{align*}

Based on above observations, $\sum_{W \in B}P(W)+\gamma <\sum_{W \in B}P(W)+b\le p$.
, which contradicts the fact that 
$$P_{d_{i+2},\vec{p}}(F)+P_{d_{i+2},\vec{p}}(T)=1.$$

Unless 

$$P_{d_{i+2},\vec{p}}(F) = a+\sum_{W \in B} P(W)+\sum_{W \in A} P(W) -(p+\epsilon-\gamma) \ge 1-p+\sum_{W \in B} P(W)-\epsilon+\gamma> 1-p.$$

Since $\sum_{W \in B} P(W) \le p$, for this inequality to be true it is necessary that $\gamma \ge \epsilon$. Thus, $P_{d_{i+2},\vec{p}}(T)\le p$
, and Theorem~\ref{bounddelegation} holds.
\end{comment}

\end{proof}


\begin{comment}
	

		From these observations, we obtain: %that $P_{H_{i+1},\vec{p}}(T)$ can be rewritten as:
		\begin{align*}
		P_{d_{i+1},\vec{p}}(T) =& P_{d_{i},\vec{p}}(T) - (1-p)\sum_{W \in B} P(W) 
		+ p\sum_{W \in A} P(W) \\
		P_{d_{i+1},\vec{p}}(F) =& P_{d_{i},\vec{p}}(F) - p\sum_{W \in A} P(W) + (1-p)\sum_{W \in B}  P(W)
		\end{align*}
%		And $P_{H_{i+1},\vec{p}}(F)$ can be expressed as:
%		\begin{align*}
		%P_{H_{i+1},\vec{p}}(F) =& P_{H_{i},\vec{p}}(F) - \sum_{W \in A_i} P(W) + \sum_{W \in A_i} P(W)(1-p) + \sum_{W \in B_i}  P(W)(1-p)
		%\end{align*}
		
		To prove Theorem~\ref{bounddelegation}, it is enough to show that:
		
        \begin{equation}\label{eqDifFandT}
          \begin{split}
		    P_{H_{i+1},\vec{p}}(T) - P_{H_{i+1},\vec{p}}(F)
		    =& P_{H_{i},\vec{p}}(T) - P_{H_{i},\vec{p}}(F) + \sum_{W \in A_i} P(W) - \sum_{W \in B_i} P(W)\\ +& (2p-1)\sum_{W \in B_i}P(W) + (2p-1)\sum_{W \in A_i} P(W)\\ \le& 2p-1.
          \end{split}
        \end{equation}
	
		
		Let $0 \le x\le p$. Then $P_{H_{i},\vec{p}}(F)= 1-x$ and $P_{H_i,\vec{p}}(T)= x$. Since $p<1/2$, in order for Equation~\ref{eqDifFandT} to be correct, we should prove that the following equation holds.
	
	    \begin{align}\label{eqDifSucandUnSuc}
		    Dif(A_i, B_i)=& \sum_{W \in A_i} P(W) - \sum_{W \in B_i} P(W) \le 1-2x.
		\end{align}
		
		Indeed, the proof of Theorem~\ref{bounddelegation} follows by Lemma~\ref{lmDifAandB}. In particular, using Lemma~\ref{lmDifAandB}, we will prove that Equation~\ref{eqDifSucandUnSuc} holds, and show that it results in Equation~\ref{eqDifFandT}.
		
		\begin{lemma}\label{lmDifAandB}
		  $Dif(A_i, B_i)\le 1-2x$, where $0 \le x \le p$.
		
		\begin{proof}
		  
	
	    We have two cases:
	     \begin{enumerate}
	        \item $\sum_{W \in B_i} P(W) \ge \sum_{W \in A_i} P(W)$.\label{caseBgreaterthanA}
	        \item $\sum_{W \in B_i} P(W) < \sum_{W \in A_i} P(W)$.\label{caseAgreaterthanB}
	     \end{enumerate}
	    In Case~\ref{caseBgreaterthanA}, obviously the lemma holds. Let us prove that the lemma is working in Case~\ref{caseAgreaterthanB}. Recall that
		
		\begin{align}\label{eqSucc}
		   P_{H_i,\vec{p}}(T)=\sum_{S \in \text{Succ}(H_i)} P[\mathcal{X}_{H_i} = S]= \sum_{S \in \text{Succ}(H_i)\setminus B_i} P[\mathcal{X}_{H_i} = S]+\sum_{W \in B_i} P(W)= x.
		\end{align}
		
		And,
		\begin{align}\label{eqUnSucc}
		   P_{H_i,\vec{p}}(F)= \sum_{S' \in \text{UnSucc}(H_i)\setminus A_i} P[\mathcal{X}_{H_i} = S']+ \sum_{W \in A_i} P(W)= 1-x.
		 \end{align}
		 
		 Hence, to prove that $Dif(A_i, B_i)\le 1-2x$ in Case~\ref{caseAgreaterthanB}, it is sufficient to show that
		
		\begin{align}\label{eqUnSuccandSucc}
		    \sum_{S \in \text{Succ}(H_i)\setminus B_i} P[\mathcal{X}_{H_i} = S] \le \sum_{S' \in \text{UnSucc}(H_i)\setminus A_i} P[\mathcal{X}_{H_i} = S'].
		\end{align}
		
		 Based on our induction hypothesis, $P_{H_i,\vec{p}}(F) > P_{H_i,\vec{p}}(T)$ and also we know that $\sum_{W \in B_i} P(W) < \sum_{W \in A_i} P(W)$. Therefore, Inequality~\ref{eqUnSuccandSucc} must hold, which concludes the proof.
		 \end{proof}
	   \end{lemma}
	 
	   
		
		
    Now, we can prove Theorem~\ref{bounddelegation}.
   \begin{proof}[Proof of Theorem~\ref{bounddelegation}]
		 Recall that to prove Theorem~\ref{bounddelegation}, it remains to show that Equation~\ref{eqDifFandT} works. By Lemma~\ref{lmDifAandB}, Equation~\ref{eqDifSucandUnSuc} holds. Recall that $0\le x\le p$. Thus
	
	\begin{equation}\label{eqDifFandTCase1}
	   \begin{split}
		 P_{H_{i+1},\vec{p}}(T) - P_{H_{i+1},\vec{p}}(F)
		 =& P_{H_{i},\vec{p}}(T) - P_{H_{i},\vec{p}}(F) + Dif(A_i, B_i) + (2p-1)\sum_{W \in B_i} P(W)+ (2p-1)\sum_{W \in A_i} P(W)\\ &\le (2p-1)(\sum_{W \in B_i} P(W)+\sum_{W \in A_i} P(W)).
      \end{split}
    \end{equation}
	
	Note that the second inequality holds, since $Dif(A_i, B_i)\le1-2x$ and 
	\begin{align*}
	    P_{H_{i},\vec{p}}(T) - P_{H_{i},\vec{p}}(F) + Dif(A_i, B_i)\le 0.
	\end{align*}

	
	
	Similarly, for the case where two new gurus $g_{i+1}$ and $g_{i+2}$ are added, one can prove that Theorem~\ref{bounddelegation} holds. In particular, let us consider $S \in Gu(H_{i+2})$ and $W = S\cap Gu(H_i)$ and $w_{i+1}=w(g_{i+1})+w(g_{i+2})$. Then, we make the following simple observations: 
    \begin{itemize}
		\item if $\lceil n_i/2\rceil \le w(W) < \lceil n_i/2\rceil + w_{i+1}/2$, then $S\in \text{Succ}(H_{i+2})$ iff $S\cap\{g_{i+1}, g_{i+2}\} \neq \emptyset$. Let $ B_i $ be the set of all the relevant subsets $ W $.
			
		\item if $ \lfloor n_i/2\rfloor \le w(W) < \lfloor n_i/2\rfloor + w_{i+1}/2$, then $S\in \text{Succ}(H_{i+1})$ iff $\{g_{i+1}, g_{i+2}\} \subseteq S$. Let $ A_i $ be the set of all the relevant subsets $ W $.
	\end{itemize}
	
So, we have 

\begin{align*}
    P_{H_{i+2},\vec{p}}(T) =& P_{H_{i},\vec{p}}(T) + \sum_{W \in B_{i}}  P(W)(p^{2}+ 2p(1-p)) + \sum_{W \in A_{i}} P(W)p^{2} - \sum_{W \in B_{i}} P(W).
\end{align*}

And,

\begin{align*}
    P_{H_{i+2},\vec{p}}(F) =& P_{H_{i},\vec{p}}(F) + (1-p)^{2}\sum_{W \in B_{i}} P(W) + ((1-p)^{2}+2p(1-p))\sum_{W \in A_{i}} P(W) - \sum_{W \in A_{i}} P(W).
\end{align*}


Now, we want to show that
\begin{equation}\label{eqDifFandTCase2}
  \begin{split}
    P_{H_{i+2},\vec{p}}(T) - P_{H_{i+2},\vec{p}}(F) =& P_{H_{i},\vec{p}}(T) - P_{H_{i},\vec{p}}(F) + \sum_{W \in A_i} P(W) - \sum_{W \in B_i} P(W)\\ +& (p^2+2p(1-p))\sum_{W \in B_i} P(W)-(1-p)^2\sum_{W \in B_i}P(W) \\+& p^2\sum_{W \in A_i} P(W)-((1-p)^2+2p(1-p))\sum_{W \in A_i} P(W)\\ \le& 2p-1.
   \end{split}
\end{equation}

By using Lemma~\ref{lmDifAandB} and replacing $\sum_{W \in A_i} P(W)$ and $\sum_{W \in B_i} P(W)$ by $1-y_1$ and $x_1$ respectively, where $x_1\le y_1 \le 1$ and $0\le x_1\le x$, Equation~\ref{eqDifFandTCase2} is rewritten as

\begin{align*}
    P_{H_{i+2},\vec{p}}(F) - P_{H_{i+2},\vec{p}}(T) \\=&P_{H_{i},\vec{p}}(T) - P_{H_{i},\vec{p}}(F) + Dif(A_i,B_i)\\ +& (4p-1-2p^2)\sum_{W \in B_i} P(W) + (2p^2-1)\sum_{W \in A_i} P(W)\\\le& (4p-1-2p^2)\sum_{W \in B_i} P(W) + (2p^2-1)\sum_{W \in A_i} P(W).
\end{align*}


\end{proof}	
   
\end{comment}




\begin{comment}
		
		
		Now, Let us analyze Equation~\ref{eqbounddelegation}, where two cases can happen:
		\begin{enumerate}
			\item $ \sum_{W \in A_i} P(W) \le \sum_{W \in B_i}  P(W) $.
			
			\item $ \sum_{W \in A_i} P(W) > \sum_{W \in B_i}  P(W) $.
		\end{enumerate}
		
		\begin{enumerate}
			\item \textit{Case 1.} In this case, obviously
			
			$$ P_{H_{i+2},\vec{p}}(T) - P_{H_{i},\vec{p}}(T) \le 0 $$
			where we have used the fact that $p < 0.5$, which concludes the proof.
			
			\item \textit{Case 2.} In this case, we can prove that $$P_{H_i,\vec{p}}(T)=\sum_{S \in \text{Succ}(H_i)} P[\mathcal{X}_{H_i} = S] \le p.$$
			
			as follows.
			
			Based on the above observations, we realize that either $W \in A_i$ or $W \in B_i$ (or both) vote in favor of the ground truth as follows.
			
			\begin{align}\label{eqground}
			p^2\sum_{W \in A_i} P(W) + (p^2 + 2p(1-p)) \sum_{W \in B_i}  P(W).
			\end{align}
			
			Also, in the favor of F as follows.
			\begin{align}\label{eqfalse}
			((1-p)^2 + 2p(1-p))\sum_{W \in A_i} P(W) + (1-p)^2  \sum_{W \in B_i}  P(W).
			\end{align}
			Since $p<0.5$, Equation~\ref{eqfalse} is greater than Equation~\ref{eqground}, which concludes the proof. 
		\end{enumerate}
		
		It is worth noting that there exists the case only one of the two new added gurus $ t_{i+1} $ and $ t_{i+2} $ (or none of them), say $ t_{i+1} $, can turn an unsuccessful set to a successful one and vice versa. Recall that $S \in Gu(H_{i})$ and $W = S\cap Gu(H_{i})$. It means that 
	\begin{enumerate}
		\item $S\in \text{Succ}(H_{i+2})$ either $\{t_{i+1}\} \subseteq S$ or $S\cap\{t_{i+1}\} = \emptyset$.\label{caseWithoutNewGuru}
		
		\item $S\in \text{Succ}(H_{i+2})$ iff $S\cap\{t_{i+1}\} \neq \emptyset$.\label{caseWithNewGuru}
		
	\end{enumerate}
	
	Obviously, in Case~\ref{caseWithoutNewGuru} the lemma holds. For Case~\ref{caseWithNewGuru}, in a similar way as above, $W \in A_i$ or $W \in B_i$ (or both) vote in favor of the ground truth as follows.
			
			\begin{align}\label{eqground2}
			p\sum_{W \in A_i} P(W) + p \sum_{W \in B_i}  P(W).
			\end{align}
			
			Also, in the favor of F as follows.
			\begin{align}\label{eqfalse2}
			(1-p)\sum_{W \in A_i} P(W) + (1-p)  \sum_{W \in B_i}  P(W).
			\end{align}
			Since $p<0.5$, Equation~\ref{eqfalse2} is greater than Equation~\ref{eqground2}. Consequently, we obtain that $P_{H_{n+2},\vec{p}}(T) \le  P_{H_{n},\vec{p}}(T) \le p_{\max}$, which concludes the proof. 
			
			\end{comment}
	
		
\begin{comment}
		%\begin{equation}\label{eqhypothesis}
		%P_{H^{*},\vec{p}}(T)=\sum_{i=\lfloor (n+2)/2\rfloor +1 }^{n+2} \binom{n+2}{i}p^{i}(1-p)^{n+2-i}\le p.
		%\end{equation}
		
		
		%Stated differently, we want to show that $P_{H^{*},\vec{p}}(T)$ is still less than or equal to $p < 1/2$, if we add two new voters $ v_{n+1} $ and $ v_{n+2} $ to the election such that $\max(p_{v_{n+1}}, p_{v_{n+2}})\le p$. Let $ V_n $ be the set of voters when the number of voters is $ n $. Let the truth set $ X_n$ denote the random variable denoting the set of gurus (voters) voting correctly. When we add two new voters, the truth set $ X_{n+2} $ is successful if  its realization set $ x_{n+2} $ is successful, which means that $|x_{n+2}|\ge \lfloor (n+2)/2\rfloor + 1$.  It is worth mentioning that after adding new voters $ v_{n+1} $ and $ v_{n+2} $, the probability of subsets $ V_n $ that have cardinality weights are either less than $ \lfloor n/2\rfloor$ or more than $ \lfloor n/2\rfloor +1$ are not changed. In particular, let $ V^{'}_n$ be the set of all the realization sets with the cardinalites of either less than $ \lfloor n/2\rfloor$ or more than $ \lfloor n/2\rfloor +1$. Obviously, they are remained successful (or unsuccessful) if either $ v_{n+1} $ or $ v_{n+2} $ (or both) cast a vote for T or F. More precisely, let $c \in V^{'}$ with the cardinality of more than $ \lfloor n/2\rfloor +1$, which is a successful realization set. So, the cardinality of $ c $ is at least $ \lfloor n/2\rfloor +3$. Let $ P(c) $ be the probability $ c $ votes for the ground truth. Let $ c^{'}= c \cup \left\lbrace v_{n+1}, v_{n+2}\right\rbrace $. If both voters either vote for T or F,
		
		%$$ P(c^{'})=P(c)\times (p^{2} + 2p(1-p)+(1-p)^{2})= P(c).$$
		
		%In the same way, we can show that if $c \in V^{'}_n$ with the cardinality of less than $ \lfloor n/2\rfloor$, by adding these two new voters, the probability it votes for F is not changed.
		
		%So, the key observation here required for the proof is the following one: by adding these two new voters $ v_{n+1} $ and $ v_{n+2} $, we can only focus on the truth sets $ X_{n} $ that can be changed from successful truth sets to unsuccessful truth sets, and vice versa. Obviously, the unsuccessful truth sets that can turn into successful ones, and vice versa, by adding these two voters are the truth sets with the realization sets of cardinality $ \lfloor n/2\rfloor$ and $ \lfloor n/2\rfloor +1$. Let $ A_n $ and $ B_n $ be the set of all the truth realization sets of cardinality $ \lfloor n/2\rfloor$ and $ \lfloor n/2\rfloor +1$, respectively.
		
		%Consider a truth realization set $ a_i \in A_n$. Before adding the two voters, $ a_i $ is an unsuccessful set, which means that voters in $ a_i $ vote with the probability of $ P(a_i)=p^{\lfloor n/2\rfloor}(1-p)^{\lfloor n/2\rfloor +1}  $ in favor of the alternative F. For every $ i\in [|A_n|] $, let $a^{'}_i=a_i \cup \left\lbrace v_{n+1}, v_{n+2} \right\rbrace $. With respect to $ P(a_i) $, in the following possible value of $ P(a^{'}_i) $ is examined.
		
		%\begin{enumerate}
		%	\item If both voters vote for T, $ a^{'}_i$ votes for the ground truth with the probability of 
		
		%	\begin{equation}\label{eqA1}
		%	P(a^{'}_i)=P(a_i)\times p^{2}=p^{\lfloor n/2\rfloor +2}(1-p)^{\lfloor n/2\rfloor +1}.
		%	\end{equation}
		
		%	\item If either $ v_{n+1} $ or $ v_{n+2}  $ votes for F, $ a^{'}_i$ votes for F with the probability of 
		
		%	\begin{equation}\label{eqA2}
		%	P(a^{'}_i)=2 \times P(a_i) p(1-p)=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor +2}.
		%	\end{equation}
		
		%	\item If both voters vote for F, $ a^{'}_i$ votes for F with the probability of 
		
		%	\begin{equation}\label{eqA3}
		%	P(a^{'}_i)= P(a_i) (1-p)^{2}=p^{\lfloor n/2\rfloor}(1-p)^{\lfloor n/2\rfloor +3}.
		%	\end{equation}
		
		%\end{enumerate}
		
		%We suppose $ A^{'}_m $ is the set of all subsets $ a^{'}_i $ that vote for the ground truth with the probability of $ P(a_i)\times p^{2} $.
		
		
		%Consider a truth realization set $b_j \in B_n$. Before adding these two voters, $ b_j $ is a successful set, which means that voters in $ b_j $ vote for T with the probability of $P(b_j)=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor}$. Let $b^{'}_j=b_j \cup \left\lbrace v_{n+1}, v_{n+2} \right\rbrace $. With respect to $ P(b_j) $, in the following possible value of $ P(b^{'}_j) $ is examined.
		
		%\begin{enumerate}
		%	\item If both voters vote for T, $ b^{'}_j$ votes for the ground truth with the probability of 
		
		%	\begin{equation}\label{eqB1}
		%	P(b^{'}_j)=P(b_j)\times p^{2}=p^{\lfloor n/2\rfloor +3}(1-p)^{\lfloor n/2\rfloor}.
		%	\end{equation}
		
		%	\item If either $ v_{n+1} $ or $ v_{n+2}  $ votes for T, $ a^{'}_i$ votes for T with the probability of 
		
		%	\begin{equation}\label{eqB2}
		%	P(a^{'}_i)=2 \times P(b_j) p(1-p)=p^{\lfloor n/2\rfloor +2}(1-p)^{\lfloor n/2\rfloor +1}.
		%	\end{equation}
		
		%	\item If both voters vote for F, $ b^{'}_j$ votes for F with the probability of 
		
		%	\begin{equation}\label{eqB3}
		%	P(b^{'}_j)=P(b_j)\times (1-p)^{2}=p^{\lfloor n/2\rfloor +1}(1-p)^{\lfloor n/2\rfloor +2}. 
		%	\end{equation}
		%\end{enumerate}
		
		%We suppose $ B^{'}_m $ is the set of all subsets $ b^{'}_j$ that vote for the alternative F with the probability of $ P(b_j)\times (1-p)^{2} $.
		
		%The number of realization sets in their relevant Equations \ref{eqA1}, \ref{eqA2} and \ref{eqA3} are equal to the number of realization sets in their relevant Equations \ref{eqB3}, \ref{eqB2} and \ref{eqB1}, respectively. So, it is enough to show that the sum of Equations \ref{eqA1}, \ref{eqB1} and \ref{eqB2} is less than the sum of Equations \ref{eqA2}, \ref{eqA3} and \ref{eqB3}. Since $ p< 1/2 $, this holds, which implies that if we add new voters $ v_{n+1} $ and $ v_{n+2} $, the probability of wining the ground truth is getting decreased. Therefore, Equation \ref{eqhypothesis} holds and this induction proves the lemma.
		\end{comment}
%\HG{End of to be removed.}
%
%
%In the same way, we can prove that $P_{H^{*},\vec{p}}(T) \le p_{max}$ when voters can delegate (i.e., liquid democracy).

\begin{comment}



\begin{proof}[Proof of Lemma~\ref{bounddelegation}]
%Let $A_n = \{ a\subseteq \Forest | w(a) \ge \lfloor m/2\rfloor +1\}$
Let $ H $ be an arbitrary delegation graph containing a forest $ \Forest = \left\lbrace t_1, t_2, ..., t_q\right\rbrace$. Let $ p=p_{max} $. We would like to show that  $ P_{H,\vec{p}}(T) \le p$. Again, by induction on the number of trees that the delegation graph $ H $ contains, we can prove that $P_{H,\vec{p}}(T) \le p$, where $ p < 1/2$. Before proving the lemma, it is useful to mention some properties of delegation graph $ H $. 

Let $ OF $ be the set of trees in $ H $ such that for each $ t \in OF $, $ w(t) $ is odd. Since the number of voters is odd, $ |OF|\ge 1 $, and obviously is odd. So, in our induction, in order to have odd number of voters at each step, we suppose that the first tree $ t_1 $ has odd numbers of voters. Also, at the other steps, we add either two trees $ t_i $ $t_{i+1}$ with cardinalites of odd, or a tree $ t_j $ with cardinality of even.  

Let $ \Forest_j$ be a forest containing $ j $ trees. Let $Q_j=2^{\Forest_j}$ denote the powerset of $ \Forest_j $. Let the truth sets $X_j$ and $ Y_j $ denote the random variables denoting the set of gurus voting correctly and incorrectly, respectively, where the number of gurus is $ j $. The number of successful subsets are equal to the number of unsuccessful ones in $ Q_j $. Because for any successful truth set $ X_j $, there is an unsuccessful truth set $ Y_j $, where $ X_j=Y_j $. $ Q_j $, and so, $ Q_j $ is called \textit{symmetric}.


So, we first sort trees in a way that for any $ i\in [q] $, $ |t_1|+|t_2|+...+|t_i| $ is odd. Let $ H_i$ denote the delegation graph containing trees $t_1, t_2, ..., t_i$ and $ n_i $ denote the number of voters $H_i$ contains. For the sake of simplicity, $ w(t_1) $ is odd. When $ q=1 $, obviously $P_{H_1,\vec{p}}(T) \le p$ and the lemma holds. Let us assume the result true for a number of gurus $q \ge 1 $. Put another way, we have, $$P_{H_q,\vec{p}}(T) \le p.$$ Consider tree $ t_{q+1} $, as we mentioned above in order to have odd number of voters in each step, two cases are considered, 

\begin{enumerate}
\item If $ w(t_{q+1}) $ is even, we insert the tree and want to prove that 

\begin{equation}\label{eqhypdelegation1}
P_{H_{q+1},\vec{p}}(T) \le p.
\end{equation}

\item If $ w(t_{q+1}) $ is odd, we also insert another tree $ t_{q+2}  $, where $ w(t_{q+2}) $ is odd, and want to prove that 

\begin{equation}\label{eqhypdelegation2}
P_{H_{q+2},\vec{p}}(T) \le p.
\end{equation}
\end{enumerate}



We prove the first case (the second case can be proved in the same way). The first case says that if we insert the tree $ t_{q+1} $ with guru $ Gu(t_{q+1}) $ and weight $ w(t_{q+1})$ to delegation graph $ H_q $, again $ P_{H_{q+1},\vec{p}}(T) \le p$. By following Lemma \ref{bound}, we can only focus on the truth sets $ X_{q} $ that can be changed from successful truth sets to unsuccessful truth sets, and vice versa. So, the relevant realization sets that their cardinalities lie in interval $ \left( n/2 - w(t_{q+1}), n/2+w(t_{q+1}) \right)$ are considered. 

Let $ A_q $ be the set of all the realization sets $ a $ of cardnality $ n_q/2-w(t_{q+1}) <|a|\le n_q/2$. Consider an unsuccessful set $ a_i \in  A_q$, it casts a vote for F with the probability of $ P(a_i)= p^{|a_i|}(1-p)^{q-|a_i|} $. For every $ a_i\in A_q$, let $a^{'}_i=a_i \cup \left\lbrace t_{q+1} \right\rbrace $. With respect to $ P(a_i) $, in the following possible value of $ P(a^{'}_i) $ is examined.

\begin{enumerate}
\item If $ t_{q+1} $ votes for T, $ a^{'}_i$ votes for the ground truth with the probability of 

\begin{equation}\label{eqAq1}
P(a^{'}_i)=P(a_i)\times p=p^{|a_i|+1}(1-p)^{q-|a_i|}.
\end{equation}



\item If $ t_{q+1} $ votes for F, $ a^{'}_i$ votes for F with the probability of 

\begin{equation}\label{eqAq2}
P(a^{'}_i)=P(a_i)\times (1-p)=p^{|a_i|}(1-p)^{q-|a_i|+1}.
\end{equation}

\end{enumerate}

Let $ B_q $ be the set of all the realization sets $ x_q $ of cardnality $ n_q/2 <|x_q|\le n_q/2+w(t_{q+1})$. Since $ Q_q $ is symmetric, for any $ a_i \in A_q$, there is a $ b_j \in B_q $, who votes with the probability of $ P(b_j)=p^{|b_j|}(1-p)^{q-|b_i|}=p^{q-|a_i|}(1-p)^{|a_i|} $ in favor of T. For every $ b_j\in B_q$, let $b^{'}_j=b_j \cup \left\lbrace t_{q+1} \right\rbrace $. With respect to $ P(b_j) $, in the following possible value of $ P(b^{'}_j) $ is examined.

\begin{enumerate}
\item If $ t_{q+1} $ votes for T, $ b^{'}_j$ votes for the ground truth with the probability of 

\begin{equation}\label{eqBq1}
P(b^{'}_j)=P(b_j)\times p=p^{|b_j|+1}(1-p)^{q-|b_j|}.
\end{equation}


\item If $ t_{q+1} $ votes for F, $ b^{'}_j$ votes for F with the probability of 

\begin{equation}\label{eqBq2}
P(b^{'}_j)=P(b_j)\times (1-p)=p^{|b_j|}(1-p)^{q-|b_j|+1}.
\end{equation}

\end{enumerate}


We know that $ a_i $ and $ b_j $ have the same cardinality. So, it is enough to show that the sum of Equations \ref{eqAq1} and \ref{eqBq1} is less than Equations \ref{eqAq2} and \ref{eqBq2}. Since $ p<1/2 $, this holds. Therefore, Equation \ref{eqhypdelegation1} holds. In the same way and by following Lemma \ref{bound}, Equation \ref{eqhypdelegation2} also holds and this induction proves the lemma.
\end{proof}

\end{comment}
%$$P_{H,\vec{p}}(T)=\sum_{\mathcal{K}}^{n}\binom{2\mathcal{K}}{\frac{\mathcal{K}}{2}}.$$

\begin{comment}
Lemma \ref{bound} suggests us the following simple algorithm:

\begin{algorithm}[H]
\caption{ ADPU }
\label{algADPU}
\hspace*{\algorithmicindent} \textbf{Input:} An undirected graph $G$, $T$ (the ground truth) and $F$.\\
\hspace*{\algorithmicindent} \textbf{Output:} $H = (V, E)\in \Delta(G)$. 
\begin{algorithmic}[1]\baselineskip=14pt\relax

\STATE Select a voter $ i $ as guru such that $ p_i=p_{max} $.
\STATE Every one delegates to i.
\end{algorithmic}
\end{algorithm}

\begin{theorem}
Algorithm \ref{algADPU} is a factor 1/2 approximation algorithm for ODPU.

\begin{proof}
Let $ H $ be the outcome of Algorithm \ref{algADPU}. Let $H^{*}$ be the optimal solution. Based on lemma \ref{bound}, if $ p_{max} < 1/2$, $P_{H^{*},\vec{p}}(T)=p_{max}$. So, in this case $P_{H^{*},\vec{p}}(T)=P_{H,\vec{p}}(T)$. Obviously, when $ p_{max} \ge 1/2 $, $ P_{H^{*},\vec{p}}(T)  \le 1$ and $ P_{H,\vec{p}}(T)=p_{max} $. So, in the worst case, $ 1/2 \times P_{H^{*},\vec{p}}(T) \le P_{H,\vec{p}}(T) $.

\end{proof}
\end{theorem}
\end{comment}

\begin{comment}
In the following we consider another version of ODPU, where we are given a delegation graph as input and we are allowed to change at most $k$ delegations to maximize the probability of the ground truth being selected. We term this problem $k$-ODPU for Optimal $k$-Delegation Problem on Undircted graph. The parameter $k$ represents a budget parameter modeling the extent to which we are able to change an initial delegation graph. $k$-ODPU is formally defined in the following way:\\

\noindent\fbox{\parbox{12.7cm}{
		\textbf{$k$-ODPU} (Optimal $ k $-Delegation Problem on Undirected graph)\\
		\emph{Input}:\ An undirected graph $G$, two alternatives $T$ (the ground truth) and $F$, a delegation graph $H = (V, E) \in \Delta(G)$, a vector of confidence levels $\vec{p}$ and a budget $k$. \\
		\emph{Feasible Solution}: A delegation graph $H^{'} = (V, E^{'})\in \Delta(G)$ s.t. $|E^{'} \setminus E|\le k$. \\
		\emph{Measure}: $P_{H^{'}, \vec{p}}(T)$ to maximize.
}}\\



\begin{theorem}\label{odpudelgation}
	$k$-ODPU is inapproximable within a factor of $\alpha \le 1$.
	
	\begin{proof}
		In the following we would like to show that $k$-ODPU is inapproximable via a reduction from the Set Cover problem, consisting of the universal set $U= \left\lbrace 1, 2, ..., n\right\rbrace  $ and set $ S=\left\lbrace S_1, S_2,..., S_m\right\rbrace  $.
		We construct a graph $ G(V, E) $ where $ V $ and $ E  $ are defined as follows(see SubFig.\ref{odpufig}. For each $ i \in U $, let $ v_{i1}, v_{i2}, ..., v_{im^{2}} , v_{i(m^{2}+1)}, ..., v_{i(2m^{2})}$ be the nodes in $ V $ such that for every $ j \in [2m^{2}-1] $, there is an undirected edge $ \left\lbrace v_{ij+1}, v_{ij} \right\rbrace $ and each voter $ v_{ij} $ has a competence level $ 0 $. For each $ S_i \in S$, let $ v_{S_i}$ be a node in $ G $, each with confidence level $0.5 \%$. For every $ i\in [n]  $ and $ j \in [m] $, there is an undirected edge $\left\lbrace  v_{i,1}, V_{S_j} \right\rbrace $ if $ i \in S_j $. For every $ i \in [n-1] $, an undirected edge $\left\lbrace v_{i, m^{2}+1}, v_{i+1, m^{2}+1}\right\rbrace $ is drawn.
		
		Consider the delegation graph $ H \in \Delta(G)$ as follows (see Fig.\ref{odpudelegationfig}). For each $ i \in [n] $ and $ j \in [m^{2}]$, voter $ v_{ij} $ delegates to $ v_{i(j-1)} $. For each $ i \in [n] $ and $ j \in [m^{2}]$, voter $ v_{ij} $ delegates to $ v_{ij-1}$. The remaining voters vote directly. We define a budget $\bar{k}=n$. Since $ nm^{2} $ voters vote for the alternative F, budget $ n $ is required for which, for every $ i \in [n] $, voter $ v_{i1} $ delegate to one of the feasible voters $ v_{S_j}, v_{S_j}, ..., v_{S_m} $ in order to have T as the winner. Hence, in the same way as we proved in Theorem \ref{ODPth}, we can show that there is no polynomial time algorithm that deals with $ K$-ODP and achieves an approximation guarantee of $\alpha \le 1$, unless $ P=NP $. 
		
		\begin{figure}[htbp]
			
			\centering
			
			\subfloat[An undirected graph.]{\label{odpufig}\includegraphics[height=6cm,width=5cm]{figures/odpu.png}} \hspace{2cm}
			\subfloat[The delegation graph.]{\label{odpudelegationfig}\includegraphics[height=6cm,width=5cm]{figures/dopudelegation.png}}
			\caption{}
			
			
			%\label{fig:1}
		\end{figure}
	\end{proof}
\end{theorem}

\begin{corollary}
	Theorem\ref{odpudelgation} implies that ODPU is as hard as $k$-ODPU, where the graph is disconnected.
\end{corollary}
\end{comment}

In the next section, we consider a simpler version of ODP, where the election does not rely on the structure of social network. The task is to allocate weights to the voters using vote vector belief to have T as the outcome with the highest probability, called the \textit{Optimal Voting Weight Allocation Problem} (OVWAP).

\section{OVWAP}

%Based on Corollary~\ref{corODPG}, the most hardest part in finding the optimal solution for ODP is organizing the delegation paths toward an optimal set of gurus (even if this set is known in advance). 

We consider another simple variant of ODP, where a set of voters and their confidence levels are given, and we are asked to allocate weights to voters in way that the ground truth is selected with high probability, without exceeding a given budget $W$.  So, the goal is to find a vector of $ \vec{w}=(w_1, w_2,..., w_n) $, where every voter $i$ has an associated weight $w_i$ and $\sum_{i}^{n} w_i=W$, to maximize $P_{\vec{w}, \vec{p}}(T)$, i.e., the ground truth's probability being chosen with respect to $\vec{w}$ and $\vec{p}$.\\

\noindent\fbox{\parbox{12.8cm}{
		\textbf{OVWAP} (Optimal Voting Weight Allocation Problem)\\
		\emph{Input:}\ Two alternatives $T$ (the ground truth) and $F$, a set of voters $V$, a vector of confidence levels $\vec{p}$ and a budget $W=n$ of voting weight.\\
		\emph{Feasible Solution}: An allocation $w: V \longrightarrow \mathbb{N}$ such that $sum_{v\in V} w(v) = n$. \\
		\emph{Measure}: $P_{\vec{w}, \vec{p}}(T)$ to maximize.
}}\\


Terzopoulou and Endriss~\cite{terzopoulou2019optimal} investigated the fractional version of the problem. They proved that the best rule is weighted majority rule and determine the optimal solution $w$ based on the voter's confidence level. 
%But in this study, its integral version (i.e., OVWAP) is NP-complete. \HG{Do you have a proof?}

We can make a link to weighted voting games. A weighted voting game $G$ with a set of players $N = \{1,\ldots,n\}$ is a cooperative game defined by a list of weights $w = (w_1,\ldots,w_n)\in \mathbb{R}^{n}$ and a quota $q \in R$; we will write $G=[N;w;q]$. The characteristic function $v: 2^{N} \rightarrow \{0,1\}$ of the game is defined as follows: $v(C)= 1$ if $\sum_{i\in C} w_i \ge q$ and $0$ otherwise.
Let us write $w(C)$ to denote the total weight of a coalition $C$. 

While weighted voting games allow for arbitrary real number weights, Brandt et al.~\cite{brandt2016handbook} note that any weighted voting game is equivalent to a game with fairly small integer weights by using a Theorem from~\cite{muroga1971threshold}.

\begin{theorem}
Let  us  say  two  weighted  voting  games $G=[N;w;q]$ and $G'=[N;w';q']$ are equivalent iff for all coalitions $C$ we have $w(C)\ge q$ iff $w'(C)\ge q'$. Then, for any weighted voting game $G = [N;w;q]$ with $|N|=n$, there exists an equivalent weighted voting game $G'=[N;w';q']$ with $w'=(w'_1,\ldots,w'_n)$ such that all $w'_i$ and $q'$ are nonnegative integers, and $w'_i=O(2^{n \log n})$.
\end{theorem}


In the following, it is shown that if voters with accuracy less than $1/2$ delegate to voters with accuracy more than or equal to $1/2$, the probability of choosing T is increased in OVWAP.

\begin{lemma}\label{lmWitoughtLowAccuracy1}
In OVWAP, if the voters with accuracy less than $1/2$ delegates to voters with accuracy greater than or equal to $1/2$, the chance that T being selected is increased.
\end{lemma}

To prove lemma~\ref{lmWitoughtLowAccuracy1}, we first prove some other lemmas.

\begin{lemma}\label{lmWitoughtLowAccuracy2}

If $p_1, p_2, ..., p_{n-1} \ge 1/2$ and $p_n < 1/2$, $P_{\vec{w}, \vec{p}}(T) > P_{\vec{w'}, \vec{p}}(T)$, where $\vec{w}=(w_1, w_2, ..., w_{n-1}+w_n, 0)$ and $\vec{w}'=(w_1, w_2, ..., w_{n-1}, w_n)$.

\begin{proof}
We suppose that $w_1, w_2, ..., w_n$ are sorted in non-increasing order and recall that $\sum^{n}_{i} w_i=n$. Let $\vec{w}_i$ be the restriction of vector $\vec{w}$ to the first $i$ voters.

\begin{align}\label{eqWitoughtLow}
P_{\vec{w}_{n-2}, \vec{p}_{n-2}}(T)=P_{\vec{w'}_{n-2}, \vec{p}_{n-2}}(T).
\end{align}

Thus the difference between the accuracy of $\vec{w}$ and $\vec{w}'$ appears when the last two voters are added to the voting process. Taking similar notations as Lemma~\ref{bounddelegation}, let $V_i=\{1, 2, ..., i\}$ be the set of first $i$ voters. Let $S \subseteq V_{n}$ and $W \subseteq S\cap V_{n-2}$. Let us suppose that both voters $n-1$ and $n$ can turn a successful set in $V_{n-2}$ to an unsuccessful one and vice versa. We have the following observations,

\begin{enumerate}
    
\item if $\lceil n_i/2\rceil \le w(W) < \lceil n_i/2\rceil + (w_{n-1}+w_n)/2$, then $S\in \text{Succ}(V_n)$ iff $S\cap\{n-1, n\} \neq \emptyset$. Let $ B_i $ be the set of all the relevant subsets $ W $.
			
\item if $ \lfloor n_i/2\rfloor \le w(W) < \lfloor n_i/2\rfloor + (w_{n-1}+w_n)/2$, then $S\in \text{Succ}(V_n)$ iff $\{n-1, n\} \subseteq S$. Let $ A_i $ be the set of all the relevant subsets $ W $.
\end{enumerate}

So, we have 

\begin{align*}
    P_{\vec{w}'_{n}, \vec{p}_n}(T) =& P_{\vec{w'}_{n-2}, \vec{p}_{n-2}}(T) + \sum_{W \in B_{n-2}}  P(W)(pp'+p(1-p')+p'(1-p))\\ +& \sum_{W \in A_{n-2}} P(W)pp' - \sum_{W \in B_{n-2}} P(W).
\end{align*}


Let us define

\begin{align*}
    Dif'=& P_{\vec{w}'_{n}, \vec{p}_n}(T) - P_{\vec{w}'_{n-2}, \vec{p}_{n-2}}(T)= \sum_{W \in B_{n-2}}  P(W)(p'+p-pp')\\ +& \sum_{W \in A_{n-2}} P(W)pp' - \sum_{W \in B_{n-2}} P(W).
\end{align*}

In a similar way, we have

\begin{align*}
    P_{\vec{w}_{n}, \vec{p}_n}(T) =& P_{\vec{w}_{n-2}, \vec{p}_{n-2}}(T) - \sum_{W \in B_{n-2}} P(W) + \sum_{W \in B_{n-2}}  P(W)p + \sum_{W \in A_{n-2}} P(W)p.
\end{align*}


Let us define

\begin{align*}
    Dif=&  P_{\vec{w}_{n}, \vec{p}_n}(T) - P_{\vec{w}_{n-2}, \vec{p}_{n-2}}(F)= P_{\vec{w}_{n-2}, \vec{p}_{n-2}}(T) - \sum_{W \in B_{n-2}} P(W) + \sum_{W \in B_{n-2}}  P(W)p + \sum_{W \in A_{n-2}} P(W)p.
\end{align*}

Since $p'<1/2$, by Equation~\ref{eqWitoughtLow}, it is obvious $Dif >Dif'$, which concludes the proof. Note that in case where only one of voters $n-1$ and $n$ can change a successful set to an unsuccessful one (and vice versa), one can use the same technique and shows that the lemma holds.
\end{proof}

\end{lemma}


\begin{comment}
\begin{obs}~\label{obsWitoughtLowAccuracy}
If $p_1, p_2, ..., p_{n-2} \ge 1/2$ and $p_{n-1}, p_{n} < 1/2$, $P_{\vec{w}, \vec{p}}(T) \ge P_{\vec{w'}, \vec{p}}(T)$, where $\vec{w}=(w_1, w_2, ..., w_{n-1}+w_n, 0)$ and $\vec{w}'=(w_1, w_2, ..., w_{n-1}, w_n)$.

\begin{proof}
By using the same technique as Lemma~\ref{lmWitoughtLowAccuracy2}, the observation can be proved.
\end{proof}
\end{obs}

We are now ready to prove Lemma~\ref{lmWitoughtLowAccuracy1}.

\begin{proof}[Proof of Lemma~\ref{lmWitoughtLowAccuracy1}]
  Let $V'=\{v'_1, v'_2, ..., v'_{n_1}\}$ denote all voters with accuracy less than $1/2$. Based on Observation~\ref{obsWitoughtLowAccuracy}, to increase the probability of selecting T, all voters in $V'$ can delegate to one of $v'_i \in V'$. According to Lemma~\ref{lmWitoughtLowAccuracy2}, delegating $v'_i$ to voter $v_j$ with $p_j \ge 1/2$ results in winning T with a higher chance, which concludes the lemma.
\end{proof}



    




%In $\vec{w}$ means that the voter with low confidence delegates to the expertise one (voter $n-1$), however in $$ 
Denoting by $z_n(i)$ the value $\binom{n}{i} p^{i}(1-p)^{n-i}$. Clearly, we have
\begin{align}\label{alignLowConf}
P_{\vec{w}'_{n}, \vec{p}_n} =& \big(\sum_{i=\lceil n/2 \rceil}^{n-2} z_{n-2}(i)\big)
+ z_{n-2}(\lceil n/2 \rceil-1) (pp'+p(1-p')+p'(1-p)) 
+ z_{n-2}(\lfloor n/2 \rfloor-1)pp'.
\end{align}

and 

\begin{align}\label{alignHighConf}
P_{\vec{w}_n, \vec{p}_n}=& \big(\sum_{i=\lceil n/2 \rceil}^{n-2} z_{n-2}(i)\big)
+ z_{n-2}(\lceil n/2 \rceil-1) p 
+ z_{n-2}(\lfloor n/2 \rfloor-1)p.
\end{align}

So, it is sufficient to prove that \text{Equation~\ref{alignLowConf}} minus \text{Equation~\ref{alignHighConf}} is less than $0$. 

\begin{align*}
P_{\vec{w}'_{n}, \vec{p}_n} - P_{\vec{w}_{n}, \vec{p}_n}\\ =& z_{n-2}(\lceil n/2 \rceil-1) (pp'+p(1-p')+p'(1-p)) + z_{n-2}(\lfloor n/2 \rfloor-1)pp'\\ -& z_{n-2}(\lceil n/2 \rceil-1) p 
- z_{n-2}(\lfloor n/2 \rfloor-1)p \\=& (p'-pp')z_{n-2}(\lceil n/2 \rceil-1) + (pp'-p) z_{n-2}(\lfloor n/2 \rfloor-1)\\=& {n-2 \choose \lfloor n/2 \rfloor-1}p^{\lceil n/2 \rceil-1}(1-p)^{\lceil n/2 \rceil-1}(2p' -1) < 0.
\end{align*}

where we have used the fact that ${n-2 \choose \lfloor n/2 \rfloor-1} = {n-2 \choose \lceil n/2 \rceil-1}$ and $p' < 0.5$. Consequently, we obtain that $P_{\vec{w}, \vec{p}}(T) > P_{\vec{w'}, \vec{p}}(T)$. In the case where $\sum^{n-2}_i w_i < w_{n-1}+w_{n}$ or $w_{n-1} < w_n$, it is easy to see that the lemma holds. 

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}


Following Brandt et al.~\cite{brandt2016handbook}, we have the following definitions,

\begin{definition}
A cooperative game, $G$, is given by a pair $G=(N, v)$, where $N$ is the set of players $\{1, 2, ..., n\}$ of the game, and $v: 2^{N} \rightarrow \mathbb{R}$ is the characteristic function of the game. 
\end{definition}

Consider $\textbf{x}=(x_1, x_2, ..., x_n) \in \mathbb{R}^{n}$, where $\sum^{n}_{i=1} x_i = v(N)$ and $\forall{i}\ x_i \ge 0$ in a cooperative game $G=(N, v)$.


\begin{definition}
The core, $\mathcal{C}(G)$, of a cooperative game $G=(N, v)$ is the set:
$\mathcal{C}(G)=\{x|\ \forall{C} \subseteq N: x(C)\ge v(C)\}$, where $x(C)=\sum_{i\in C} x_i$
\end{definition}

Consider a game $G$ with $N=\{1, 2, ..., n\}$ and the characteristic function $v$ defined as follows:

\begin{align}\label{lbrecursiveformula}
v(C) = \left\{ \begin{array}{c c}
W_C & \quad \text{ if } |C| > n/2  \\
0 & \quad \text{ otherwise.}\\
\end{array} \right.
\end{align}

$W_C$ is obtained in the following way. Let $\textbf{x}^{f}=(x^{f}_1, x^{f}_2, ..., x^{f}_n)$ be the optimal fractional weight, which means that $x^{f}_i=\log(p_i/(1-p_i))$. We suppose that for every voter $i$, $1/2 \le p_i < 1$. We normalize \HG{Between $0$ and $1$?} the weights and store it in $\textbf{x}^{norm}=(x^{norm}_1, x^{norm}_2, ..., x^{norm}_n)$. For any set $C \subseteq N$, we set $W_{C}=n\sum_{i\in C} x^{norm}_i$, which is the weight of coalition $C$ in the optimal fractional version of OVWAP.

There is a close connection between OVWAP and finding $\mathcal{C}(G)$, the core of the game $G$. Indeed, $\mathcal{C}(G)$ is the set of all possible optimum weight assignments, which will maximize $P_{\vec{w}, \vec{p}}(T)$ \HG{I think this is false. For instance, consider the instance with $\vec{p} = (0.5,0.5,1)$, then after normalizing the weights received in the optimal case are $(0,0,3)$. But $(0,1,2)$ is optimal but is not in the core. You even show it in your example}. So, the integer weight assignments in $\mathcal{C}(G)$ are the optimal solutions to OVWAP. Let us to give an example to make it clear. 

\begin{exmp}\label{exmpNonEmptyCore}
Consider $3$ voters $N=\{1, 2, 3\}$ with confidence levels $\vec{p}=(.55, .60, .70)$. The optimum weight is $\textbf{x}^{f}=(.0872, .1761, .3680)$, which can be normalized, $\textbf{x}^{norm}=(.138, .279, .583)$. Consider four coalitions $ C_1=\{3\}, C_2=\{1, 3\}, C_3=\{2, 3\}$ and $C_4=\{1, 2, 3\}$, which have enough weight to elect T. So, in game $G=(N, v)$ as explained above, we have $v(C_1)=1.749, v(C_2)=2.34, v(C_3)=2.01$ and $v(C_4)=3$. $\textbf{x}=(x_1, x_2, x_3)$ can be in $\mathcal{C}(G)$ if it satisfies the following constraints:

\begin{align*}
    x_1+x_2+x_3=3\\
    x_3 \ge 1.749\\
    x_1+x_3 \ge 2.34\\
    x_2+x_3 \ge 2.01
\end{align*}

Obviously, an integer solution that satisfies the above constraints is an optimal solution to OVWAP. In this case, the only optimum integer weight assignment in $\mathcal{C}(G)$ is $\textbf{x}=(0, 0, 3)$. We should mention that there are two other optimum weight assignments $\textbf{x}=(1, 0, 2)$ and $\textbf{x}=(0, 1, 2)$, which are not in the core.
\end{exmp}

Note that for some examples the core of game $G$ may be empty. \HG{Yes but not in your case. You may not have integer valued vectors but you always have at least one real vector.}

\begin{exmp}\label{exmpEmptyCore}
Consider $5$ voters $N=\{1, 2, ..., 5\}$ with confidence levels $\vec{p}=(.9, .9, .6, .6, .6)$. By going through the same process as Example~\ref{exmpNonEmptyCore}, the following constraints can be achieved:

\begin{align*}
    x_1+x_2+x_3+x_4+x_5=5\\
    x_1+x_2 \ge 3.92\\
    x_1+x_3 +x_4 \ge 2.68\\
    x_1+x_3 +x_5 \ge 2.68\\
    x_1+x_4 +x_5 \ge 2.68\\
    x_2+x_3 +x_4 \ge 2.68\\
    x_2+x_3 +x_5 \ge 2.68\\
    x_2+x_4 +x_5 \ge 2.68\\
\end{align*}
Note that we did not bring the corresponding constraints of all possible coalitions that can elect T, which are not necessaries since they do not provide any new constraint to be concerned about here. There are three optimum integer weight assignments $\textbf{x}=(2, 2, 1, 0, 0), \textbf{x}=(2, 2, 0, 1, 0)$ and $\textbf{x}=(2, 2, 0, 0, 1)$, which none of them are in $\mathcal{C}(G)$ and can satisfy all the above constraints.
\end{exmp}

\HG{I am note sure checking for an $\epsilon$ relaxation of the core is meaningful, mostly because the objective function we are looking at is not continuous but you can continue looking at this concepts if your interested. However, I am also not sure this ``core-relationship'' helps. I mean with an exponential number of contrainsts, it is easy to write an IP which solves our problem.}
\begin{definition}
$\textbf{x}$ is in the $\epsilon$-core of a game $G$, $\epsilon(G)$, if for any $C\subseteq N$, $x(C)\ge x(v) -\epsilon$ for some $\epsilon \in \textbf{R}$~\cite{chalkiadakis2011computational}.
\end{definition}

We can find the $\epsilon$-core for game $G$ that satisfies the constraints in Example~\ref{exmpEmptyCore}. But such a weight assignment may not be the optimal solutions for OVWAP. For example, for $\epsilon=1$, there is the weight assignment $\textbf{x}=(2, 1, 1, 1, 0)$, which is not an optimum assignment. Thus, it is required to check all the assignments in $\epsilon(G)$ to determine the optimum one(s), which in this case we have three optimum integer assignments as we mentioned in Example~\ref{exmpEmptyCore}. Also, in order to minimize the space of solutions, we can have the following constraints~\cite{chalkiadakis2011computational}:



\begin{align}
\begin{array}{c}
    \min \epsilon \hspace{3cm} \vspace{.3cm}\\
    \sum_{i\in N} x_i=v(N)\hspace{1.3cm} \vspace{.3cm}\\
    \hspace{1.8cm}\sum_{i \in C} x_i \ge v(C)-\epsilon \quad \text{for each} C\in N
\end{array}
\end{align}

Chalkiadakis et al.~\cite{chalkiadakis2011computational} note that there exist $2^{n}+n+1$ constraints in order to find the core of a game and we need an efficient separation oracle to check in polynomial time whether the core is non-empty. Indeed, the separation oracle outputs all weight assignments in the core, otherwise it reports all the violated constraints.
\end{comment}

==> contribution/ofdp.tex <==
\section{OFDP}

In this section, we deal with fractional version of ODP, where every voter is allowed to delegate a fraction of her power (vote) to another voter. We term this problem, OFDP, for Optimal Fractional Delegation Problem. We then present a network flow (in particular, circulation with demands) based optimal solution to the problem for the special case, where whether the weight assignment we give to each voter is feasible (we will talk about this problem at length in this section).  

Recall that coordinating voters' powers (votes) and maximizing the probability that the ground truth being selected is the goal in this version. Assuming $P\ne NP$, one can show that OFDP as ODP is inapproximable within a factor of $\alpha\le 1$.

\begin{theorem}
    OFDP is inapproximable within a factor of $\alpha \le 1$, assuming $P\ne NP$.
    \begin{proof}
    Following exactly the same reduction as Theorem~\ref{ODPth}.
    \end{proof}
\end{theorem}

We now provide a polynomial time algorithm for the special case of OFDP, where whether there exists a feasible delegation graph that results in a weight vector, that is given in advance. We term this problem \textbf{FEASDEL}. In particular, we are given a graph $G=(V, E)$ and a weight vector $\Vec{w}$ defined by $\Vec{w}[i]=w_i$, where $w_i$ representing the weight assignment we assign to voter $i$. The goal is to find a delegation graph $H$ in which for each voter $i$, $w_i=w^{out}-w^{in}_i$, where $w^{out}$ and $w^{in}_i$ denote the total weight $i$ receives and sends out, respectively. More formally,\\

\noindent\fbox{\parbox{12.7cm}{
		\textbf{FEASDEL}\\
		\emph{Input}: A social network $G$, a weight vector $\vec{w}$.\\
		\emph{Feasible Solution}: A delegation graph $H = (V, E)\in \Delta(G)$, where for each voter $i$, $w_i=w^{out}-w^{in}_i$.
}}\\

There is a one-to-one correspondence between the feasible delegation graph for a given weight vector and the problem of \textit{circulation with demands}~\cite{kleingbergalgdesign}. In the problem of circulation with demands, we are given a flow network $G=(V, E)$. For every $e$, $c_e$ represents the capacity of edge $e$. A demand $d_v$ is assigned to each vertex $v\in V$. If $d_v>0$, $v$ has a demand of $d_v$ (i.e., it is a sink) and wishes to receive $d_v$ units more flow than it sends out. If $d_v < 0$, $v$ has a supply of $-d_v$ (i.e., it is a source) and wishes to send out $-d_v$ units more flow than it receives. The node $v$ is neither source or sink otherwise ($d_v=0$). The goal here is to find a \textit{circulation} with demands $\{ d_v \}$, that is a function $f$ assigning a non-negative real number to each edge and meets the following two conditions. Let $f^{in} (v)$ and $f^{out} (v)$ denote the total weight $v$ receives and sends out, respectively.

\begin{enumerate}
    \item (Capacity conditions) For each $e \in E$, $0\le f(e) \le c_e$.\label{lbcapacity}
    
    \item (Demand conditions) For each $v\in V$, $f^{in} (v)-f^{out} (v)=d_v$.\label{lbcondition}
    
\end{enumerate}

So, the goal here is to figure out whether there exists a \textit{feasible circulation} that satisfies both conditions~\ref{lbcapacity} and~\ref{lbcondition}. One of the way to check whether a feasible circulation exists is that the following condition holds.

\begin{lemma}\label{lmfeasiblecirculation}
If there exists a feasible circulation with demands $\{ d_v\}$, then $\sum_{v\in V} d_v=0$~\cite{kleingbergalgdesign}.
\end{lemma}


We present a reduction from \textbf{FEASDEL} to the problem of finding a feasible circulation with demands $\{ d_v\}$. We show that if there exists a feasible circulation in the resulting graph, the feasible solution to \textbf{FEASDEL} can be found in polynomial time. The basic idea behind the reduction is to assign each vertex $i$ a demand $d_i= w_i - 1/n$. Recall that each voter has a weight $1/n$ in hand (weights are normalized). So, if $ w_i < 1/n$, then voter $i$ is source and wishes to delegate some of her weight to other voters through delegations. If $ w_i > 1/n$, voter $i$ is a sink and wishes to receive some weight along some delegations. Otherwise, $i$ is neither source nor sink. Each edge $e$ is associated with a large enough weight $c_e$. 
 
 \begin{obs}\label{obsfeasiblecirculation}
 If there exists a feasible circulation with demands $\{d_i\}$ (i.e., $\sum_{i \in V} d_i=0$~\ref{lmfeasiblecirculation}), then there exists a feasible delegation graph, where the weight of each voter $i$ equals $w_i$.
 
 \begin{proof}
 By following Lemma~\ref{lmfeasiblecirculation}, the proof is straight forward.
 \end{proof}
 \end{obs}
 
 We note that the problem of finding a feasible circulation with demands $\{d_v\}$ is equivalent to the problem of finding a maximum $s-t$. Hence it is polynomially solvable.
 
\begin{theorem}
     If there exists a feasible circulation in the resulting graph $G$, \textbf{FEASDEL} is solvable in polynomial time.
\end{theorem}

%It is worth noting that finding a feasible solution to \textbf{FEASDEL} enables us to figure out whether there exists a coordination of delegations to give our desire voters enough power.

==> problem/ProblemDefinition.tex <==
\section{Problem Definition}\label{secpd}

%We consider elections with two alternatives or candidates a \textit{ground truth} \textit{T} (a correct answer) and \textit{F} (a wrong answer). Let $  V= \left\lbrace 1, 2, ..., n \right\rbrace$ be a finite set of voters that take part in a vote. For the sake of simplicity, we assume the number of voters is odd. Moreover, we will often assume that the presence of a Social Network (SN) as a graph $ G=(V, E) $,\ where each node in the graph corresponds to a voter $i \in V$ and an edge $ \left(i, j\right) \in E $ corresponds to a social relation between $ i $ and $ j $. The set of neighbors of voter $ i $ is $ \Gamma (i)= \left\lbrace j \in V | \left(i, j\right) \in E \right\rbrace $. 

%In this setting, every voter $i$ has an associated confidence level $p_i$, indicating the probability that she votes for T when she decides to vote directly. We denote by $\vec{p}_V$ the vote belief vector defined by $\vec{p}_V[i] = p_i$ on the set of voters $V$. Each voter $ i $ has two possible choices: (\textit{i}) either she can vote directly, or (\textit{ii}) delegate to one of her neighbors in $ \Gamma (i) $ .\ In the first case and second case, we call the voter a \textit{guru}, and a \textit{follower}, respectively. In this model, we assume that voters do not abstain. We will use the following SN as a running example to make the concepts and problems clearer.

%\begin{exmp}\label{probex}
%	We consider an example of election with two alternatives, \textit{T} and \textit{F} and $7$ voters which are part of a Social Network (SN).\ Fig.~\ref{socialpro} shows the corresponding SN and the competence levels of the agents which are given next to them.\ Every voter $ i \in \left\lbrace 1, 2, ..., 7 \right\rbrace$ has a competency level $ p_i $, indicating the probability that she will cast a vote for T when she intends to vote directly.
	
%	\begin{figure}[htbp]
%		\centering
%		\includegraphics[scale=.2]{K-ODP/figures/socialpro.png} 
%		\caption{The SN and voter's competency levels.}
%		\label{socialpro}
%	\end{figure}
%\end{exmp}

%A \textit{delegation function} is a function $ d: V \rightarrow V $ such that: 
%\begin{itemize}
%	\item $ d(i)=j$ if voter $ i $ wants to delegate to voter $ j \in \Gamma(i)$,
%	\item $d(i)=i$ if voter $i$ has intention to vote,
	%\item $d(i) = 0$ if voter $i$ has intention to abstain.
%\end{itemize}

%We can apply a delegation function $d$ on the SN $ G $ to obtain a delegation graph $H[V]$ on the set $V$. More precisely, $H[V]$ is a subgraph of $G$ where there is an edge $(i,j)$ if voter $i$ delegates to voter $j$ and nodes with outdegree 0 are the voters who vote directly (i.e., gurus).

%Consider the following delegation function, that applies on our running example (Example~\ref{probex}). Voter $2$ delegates her vote to voter $1$, i.e., $d(2) = 1$. Voter $3$ delegates to voter $ 5 $, i.e., $d(3)=5$. Also, voter $6$ delegates to voter $ 7 $ ($d(6)= 7$). Voters $1, 4$ and $5$ vote directly, i.e., $d(1)=1, d(4)=4$ and $d(5)=5$. So, voters $ 2,3, 5 $ and $ 6 $ are the followers, and voters $ 1, 4 $ and $ 7 $ are gurus. By applying this delegation function to the SN graph $G$ represented in Fig.~\ref{socialpro}, we obtain the delegation graph $H$ shown in Fig.~\ref{delegationpro}. 

\begin{figure}[htbp]
	\centering
	\includegraphics[scale=.2]{figures/delegationgraphpro.png} 
	\caption{The delegation graph.}
	\label{delegationpro}
\end{figure}


We denote by $ \Delta (G) $ the set of \textit{delegation graphs} that can be obtained from $G$. We sometimes write $H$ instead of $H[V]$.
%It is worth noting that delegations are transferred in the edges of $G$. We denote by $H \in \Delta (G)$ a delegation graph. 
We refer to a delegation graph that has no cycle as a \textit{consistent delegation graph}.

As we mentioned, applying a delegation function on a graph $ G$ results in a delegation graph $ H$ which includes a set of gurus. More formally, we are given a forest $\Forest = \{t_1,\ldots,t_q\}$, where $t_1,\ldots,t_q$ are the trees induced by $H$ (see Fig.~\ref{delegationpro}). We denote the guru of tree $t_i \in \Forest$, and the probability she casts a vote for T by $Gu(t_i)$ and $P(t_i)$ (i.e., $P(t_i)=P(Gu(t_i))$), respectively. Let $V_{t_i}$ and $E_{t_i}$ the set of nodes and arcs in $t_i$, respectively. Each $t_i$ is assigned a weight $w(t_i) = |V_{t_i}|$ (i.e., the voting power $Gu(t_i)$ receives from herself and her followers). We also extend this notation to subsets of trees by letting $w(a) = \sum_{t\in a} w(t)$, where $a\subseteq \Forest$. Throughout the paper, we will use the weighted plurality rule. So, let $A = \{ a\subseteq \Forest | w(a) \ge (n+1)/2\}$ be the set of all subsets of $\Forest$ which have enough weight to win the election. We denote the probability that the gurus voting for $T$ are exactly the ones corresponding to the subset $a$ by $ P(a)=\prod_{t \in a}P(t) \prod_{t \notin a} (1-P(t))$. We denote by $P_{H,\vec{p}}(T)$ the probability of electing $ T $ as a winner in the delegation graph $ H $ with respect to $\vec{p}$. As a result,
$$P_{H,\vec{p}}(T) = \sum_{i=1}^{|A|} P(a_i).$$

In the example represented in Fig.~\ref{delegationpro}, T wins when either both voters $1$ and $5$, both voters $1$ and $7$, or both voters $5$ and $7$ (or all of them) vote for it. We get $P_{H,\vec{p}}(T) = 85\%$.
